Can We Trust the Teacher? Decoupled Credit Direction-Magnitude for Self-Distillation

RLVR provides reliable trajectory-level credit, while OPSD offers dense supervision for token-level credit. This exposes a fundamental coupling when updating step-level credit direction and magnitude with teacher supervision, preventing steps from receiving reliable credit directions and contribution magnitudes, while making both vulnerable to teacher judgment errors and preference variance, as supported by our theoretical analysis. To separate credit direction from its contribution magnitude, we introduce \textit{Decoupled Credit Self-Distillation (DCSD)}, which theoretically decouples credit direction and magnitude into two reliable signals and uses them to calibrate privileged teacher supervision. Specifically, we design belief-margin probing to determine credit direction and marginal information gain to quantify credit magnitude, enabling step-to-token credit assignment for policy optimization. Across 11 benchmarks, DCSD achieves the best overall scores against GRPO, OPSD, RLSD, and RLCSD. Compared with base models, DCSD improves the overall score by 8.45 points on mathematical reasoning and 7.01 points on multimodal reasoning, while correcting the credit direction for 6\% of tokens and yielding a 1.5$\times$ reduction in token credit magnitude.

==> case_01.tex <==
% Generated from immutable V2 scored JSON. Native text, not an image.
\begingroup
\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt}
\CSCaseTitle{Case 1: an incorrect angle reduction receives opposite credit}
\CSMeta{\textbf{Question:} A square and a regular heptagon share side AD. Find angle BAC as a common fraction (see the original diagram).}
\CSMeta{\textbf{Ground truth:} 270/7 degrees}
\CSLegend
\CSMeta{Same frozen response, gold-answer hint, and Base student reference.}
\CSRule
\CSModel{OPSD}{+0.005286}{positive}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{F1C1C1}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}F}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}at}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}k}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{*(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F6D8D8}{2}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{*}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{*(}\CSGap%
\CSToken{F9E5E5}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}=}\CSGap%
\CSToken{EBA8A8}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE7E7}{*(}\CSGap%
\CSToken{EDB2B2}{7}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F9E6E6}{*(}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F9E4E4}{))}\CSGap%
\CSToken{EFB9B9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Therefore}\CSGap%
\CSToken{F4CFCF}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}coordinates}\CSGap%
\CSToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}A}\CSGap%
\CSToken{F5D5D5}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}e}\CSGap%
\CSToken{F9E5E5}{\textasciicircum{}(}\CSGap%
\CSToken{FAE7E7}{i}\CSGap%
\CSToken{E17D7D}{*}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{)}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}=}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE8E8}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{EAA5A5}{)}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{EAA5A5}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E17D7D}{)\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{62AC80}{Similarly}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}for}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}others}\CSGap%
\CSToken{F4CDCD}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}equal}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}to}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F9E6E6}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}so}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}cos}\CSGap%
\CSToken{F8DFDF}{(}\CSGap%
\CSToken{EAA1A1}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE8E8}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE8E8}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE8E8}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E17D7D}{).\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E9A0A0}{Similarly}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}point}\CSGap%
\CSToken{F0BDBD}{\textperiodcentered{}B}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE8E8}{i}\CSGap%
\CSToken{F3CACA}{*}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F7DBDB}{)}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}=}\CSGap%
\CSToken{EBA7A7}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE8E8}{1}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E48686}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{CAE3D4}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE8E8}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{F7DADA}{\textperiodcentered{}-}\CSGap%
\CSToken{F5D2D2}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{).\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{EAA1A1}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}F}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F9E5E5}{*}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F4D0D0}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE7E7}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F3CACA}{*(}\CSGap%
\CSToken{E17D7D}{2}\CSGap%
\CSToken{EBA5A5}{\ensuremath{\pi}}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}-}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F8E1E1}{/}\CSGap%
\CSToken{FAE8E8}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F8DFDF}{))}\CSGap%
\CSToken{F7DDDD}{\textperiodcentered{}=}\CSGap%
\CSToken{F5D3D3}{\textperiodcentered{}e}\CSGap%
\CSToken{EDAEAE}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F1C3C3}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F1C2C2}{)}\CSGap%
\CSToken{E89C9C}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}cos}\CSGap%
\CSToken{62AC80}{(-}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F1C1C1}{).\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{EBA7A7}{Therefore}\CSGap%
\CSToken{E89C9C}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}coordinates}\CSGap%
\CSToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E48787}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}A}\CSGap%
\CSToken{E69191}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(-}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE7E7}{(}\CSGap%
\CSToken{F7DDDD}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E17D7D}{))\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}B}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}(-}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F6D7D7}{))\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F9E3E3}{Point}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}F}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{),}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F8E1E1}{))\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSModel{DCSD}{-0.015295}{negative}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E4F1E9}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}F}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}at}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}k}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{*(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F2C5C5}{2}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{*}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{*(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{FAE9E9}{*(}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{1}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{FAE9E9}{*(}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{FAE8E8}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}coordinates}\CSGap%
\CSToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E89C9C}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}A}\CSGap%
\CSToken{F9E7E7}{:}\CSGap%
\CSToken{F0BDBD}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE7E7}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F3CBCB}{*}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{87BF9E}{)}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}=}\CSGap%
\CSToken{D6E9DE}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F8E1E1}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}sin}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E17D7D}{)\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Similarly}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}for}\CSGap%
\CSToken{E89B9B}{\textperiodcentered{}others}\CSGap%
\CSToken{F9E4E4}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{EFB8B8}{But}\CSGap%
\CSToken{F3CCCC}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{EFBBBB}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}equal}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E2F0E8}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}so}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}cos}\CSGap%
\CSToken{F8E1E1}{(}\CSGap%
\CSToken{ADD3BD}{1}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{DDEDE4}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E4F1E9}{),}\CSGap%
\CSToken{F3CCCC}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{62AC80}{).\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F9E6E6}{Similarly}\CSGap%
\CSToken{EEB3B3}{,}\CSGap%
\CSToken{99C8AC}{\textperiodcentered{}point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}B}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE7E7}{*}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F5D4D4}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{62AC80}{).\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{E3F0E9}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}F}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{*}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E1EFE7}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}e}\CSGap%
\CSToken{FAE9E9}{\textasciicircum{}(}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE8E8}{*(}\CSGap%
\CSToken{DEEDE4}{2}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{E5F1EA}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{))}\CSGap%
\CSToken{E2F0E7}{\textperiodcentered{}=}\CSGap%
\CSToken{F5D1D1}{\textperiodcentered{}e}\CSGap%
\CSToken{F7DADA}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{E4F1E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F6D9D9}{)}\CSGap%
\CSToken{DFEEE5}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}cos}\CSGap%
\CSToken{E17D7D}{(-}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}sin}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE8E8}{).\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E17D7D}{Therefore}\CSGap%
\CSToken{F7DDDD}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}coordinates}\CSGap%
\CSToken{F8DEDE}{:\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}A}\CSGap%
\CSToken{E5F1EA}{:}\CSGap%
\CSToken{E38383}{\textperiodcentered{}(-}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{EBA7A7}{))\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E5F1EA}{Point}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}B}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(-}\CSGap%
\CSToken{F0F1F2}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE7E7}{))\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{FAE9E9}{Point}\CSGap%
\CSToken{F3CCCC}{\textperiodcentered{}F}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{cos}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{sin}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F9E4E4}{))\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSMeta{\textbf{The boxed step is incorrect: 23pi/14 = 2pi - 5pi/14, not 2pi - pi/14. OPSD gives positive mean credit; DCSD gives negative mean credit.}}
\CSMeta{Signal = model(+gold) log-probability minus the same Base(no-answer) log-probability. Colors encode the signal, not mathematical correctness.}
\CSSource{math500\_0166\_s3; context tokens [9859, 10242); boxed tokens [10108, 10179). Selected local case, not an overall performance estimate.}
\endgroup


==> case_02.tex <==
% Generated from immutable V2 scored JSON. Native text, not an image.
\begingroup
\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt}
\CSCaseTitle{Case 2: a correct complex-number step receives opposite credit}
\CSMeta{\textbf{Question:} William Sydney Porter tried to compute (-3 + 4i)/(1 + 2i), but omitted the minus sign and obtained 11/5 - (2/5)i. What answer should he have obtained?}
\CSMeta{\textbf{Ground truth:} 1 + 2i}
\CSLegend
\CSMeta{Same frozen response, gold-answer hint, and Base student reference.}
\CSRule
\CSModel{OPSD}{-0.066991}{negative}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E17D7D}{So}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}combining}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}all}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}those}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}terms}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{E38484}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{EAA1A1}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Combine}\CSGap%
\CSToken{E79797}{\textperiodcentered{}like}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}terms}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{DFEEE5}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}real}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}parts}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}are}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{E27F7F}{\textperiodcentered{}and}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E99D9D}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}The}\CSGap%
\CSToken{ECAAAA}{\textperiodcentered{}imaginary}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}parts}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}are}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E28181}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{So}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}first}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}let}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}compute}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}imaginary}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}parts}\CSGap%
\CSToken{EEB3B3}{:}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}}\CSGap%
\CSToken{FAE7E7}{6}\CSGap%
\CSToken{F9E4E4}{i}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{EEB6B6}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{A9D1BA}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F8E1E1}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Then}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{F4D1D1}{\textperiodcentered{}real}\CSGap%
\CSToken{EBA8A8}{\textperiodcentered{}parts}\CSGap%
\CSToken{F1C1C1}{:}\CSGap%
\CSToken{F2C7C7}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{F9E6E6}{i}\CSGap%
\CSToken{F8DFDF}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{EEB2B2}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}i}\CSGap%
\CSToken{F3C8C8}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{EDAEAE}{,}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}so}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{E17D7D}{i}\CSGap%
\CSToken{F8E0E0}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{E17D7D}{*(-}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{E17D7D}{)}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}=}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F6D8D8}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}real}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}part}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{F5D2D2}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{F7DBDB}{\textperiodcentered{}=}\CSGap%
\CSToken{E48989}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{62AC80}{Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{EEB3B3}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}numerator}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}simpl}\CSGap%
\CSToken{FAE9E9}{ifies}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}to}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{62AC80}{Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{F5D1D1}{\textperiodcentered{}the}\CSGap%
\CSToken{E58D8D}{\textperiodcentered{}entire}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}expression}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{F4CDCD}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{F5D2D2}{)/}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{E17D7D}{Div}\CSGap%
\CSToken{F7DBDB}{iding}\CSGap%
\CSToken{A2CDB4}{\textperiodcentered{}each}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}term}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}by}\CSGap%
\CSToken{E89B9B}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{F7DCDC}{i}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{F8DEDE}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{BBDBC8}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E17D7D}{Wait}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}be}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}result}\CSGap%
\CSToken{E17D7D}{?}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}seems}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}too}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}simple}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Let}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}check}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}my}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}calculations}\CSGap%
\CSToken{F6D9D9}{\textperiodcentered{}again}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}because}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}William}\CSGap%
\CSToken{E17D7D}{'s}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}incorrect}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}answer}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}was}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{/}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{/}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}i}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}which}\CSGap%
\CSToken{E99C9C}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}different}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}from}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE8E8}{1}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE7E7}{2}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Let}\CSGap%
\CSToken{EFBBBB}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}check}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}my}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}steps}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}again}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{First}\CSGap%
\CSToken{F6D9D9}{,}\CSGap%
\CSToken{8BC1A1}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}denominator}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{F3CACA}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{FAE9E9}{)(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E17D7D}{)}\CSGap%
\CSToken{89C09F}{\textperiodcentered{}=}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}-}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE8E8}{i}\CSGap%
\CSToken{FAE9E9}{)\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F2C5C5}{i}\CSGap%
\CSToken{E17D7D}{\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F1C2C2}{*(-}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE8E8}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}That}\CSGap%
\CSToken{E17D7D}{'s}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}correct}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSModel{DCSD}{+0.037267}{positive}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E17D7D}{So}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}combining}\CSGap%
\CSToken{D4E8DC}{\textperiodcentered{}all}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}those}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}terms}\CSGap%
\CSToken{62AC80}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F7DEDE}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{E17D7D}{\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{62AC80}{Combine}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}like}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}terms}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{DFEEE5}{\textperiodcentered{}real}\CSGap%
\CSToken{E2F0E8}{\textperiodcentered{}parts}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}are}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}and}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{72B48D}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{E17D7D}{\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{62AC80}{.}\CSGap%
\CSToken{E4F0E9}{\textperiodcentered{}The}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}imaginary}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}parts}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}are}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{B8D9C5}{\textperiodcentered{}+}\CSGap%
\CSToken{ECACAC}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{So}\CSGap%
\CSToken{D9EBE0}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}first}\CSGap%
\CSToken{DCECE3}{,}\CSGap%
\CSToken{E99D9D}{\textperiodcentered{}let}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}me}\CSGap%
\CSToken{BDDCCA}{\textperiodcentered{}compute}\CSGap%
\CSToken{68AF85}{\textperiodcentered{}the}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}imaginary}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}parts}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{EAA3A3}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{BCDBC8}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E99C9C}{Then}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}real}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}parts}\CSGap%
\CSToken{E5F1EA}{:}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{FAE7E7}{\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E5F1EA}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{D7EADE}{\textperiodcentered{}i}\CSGap%
\CSToken{FAE7E7}{\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}is}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}so}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F6D7D7}{i}\CSGap%
\CSToken{F9E7E7}{\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}is}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{E4F1E9}{*(-}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{E4F1E9}{)}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{BEDCCA}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{E5F1EA}{,}\CSGap%
\CSToken{BADAC7}{\textperiodcentered{}the}\CSGap%
\CSToken{E4F0E9}{\textperiodcentered{}real}\CSGap%
\CSToken{68AF85}{\textperiodcentered{}part}\CSGap%
\CSToken{EAA4A4}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F4D0D0}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}=}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{62AC80}{.}\CSGap%
\CSToken{D1E6DA}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{DBECE2}{\textperiodcentered{}the}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}numerator}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}simpl}\CSGap%
\CSToken{F0F1F2}{ifies}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{73B48D}{.}\CSGap%
\CSToken{AFD4BE}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Therefore}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{D7EADF}{\textperiodcentered{}the}\CSGap%
\CSToken{DCECE2}{\textperiodcentered{}entire}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}expression}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{FAE9E9}{)/}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{D1E6DA}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{C4DFCF}{Div}\CSGap%
\CSToken{95C6A9}{iding}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}each}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}term}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}by}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{E4F0E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}+}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{E3F0E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{A7D0B8}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E17D7D}{Wait}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}so}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}be}\CSGap%
\CSToken{86BF9D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}result}\CSGap%
\CSToken{E17D7D}{?}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}seems}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}too}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}simple}\CSGap%
\CSToken{DFEEE5}{.}\CSGap%
\CSToken{F4CDCD}{\textperiodcentered{}Let}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}me}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}check}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}my}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}calculations}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}again}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{EEB4B4}{\textperiodcentered{}because}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}William}\CSGap%
\CSToken{62AC80}{'s}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}incorrect}\CSGap%
\CSToken{F5D1D1}{\textperiodcentered{}answer}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}was}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{/}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E5F1EA}{/}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}i}\CSGap%
\CSToken{E79494}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}which}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}is}\CSGap%
\CSToken{F4CFCF}{\textperiodcentered{}different}\CSGap%
\CSToken{F1C1C1}{\textperiodcentered{}from}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{B6D8C4}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Let}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}check}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}my}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}steps}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}again}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{First}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}denominator}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{EEB4B4}{\textperiodcentered{}(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{FAE9E9}{)(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{BBDBC8}{)}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F2C8C8}{\textperiodcentered{}-}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}(}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{i}\CSGap%
\CSToken{F0F1F2}{)\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F6D6D6}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{i}\CSGap%
\CSToken{E17D7D}{\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F0BDBD}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F2C6C6}{*(-}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{E5F1EA}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}That}\CSGap%
\CSToken{62AC80}{'s}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}correct}\CSGap%
\CSToken{F0BBBB}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSMeta{\textbf{The boxed sentence is correct: (5 + 10i)/5 = 1 + 2i. OPSD gives negative mean credit; DCSD gives positive mean credit.}}
\CSMeta{Signal = model(+gold) log-probability minus the same Base(no-answer) log-probability. Colors encode the signal, not mathematical correctness.}
\CSSource{math500\_0373\_s1; context tokens [473, 785); boxed tokens [640, 668). Selected local case, not an overall performance estimate.}
\endgroup


==> case_03.tex <==
% Generated from immutable V2 scored JSON. Native text, not an image.
\begingroup
\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt}
\CSCaseTitle{Case 3: a correct annulus area receives opposite credit}
\CSMeta{\textbf{Question:} Three concentric circles have radii 4, 6, and 7. Find the difference between the greatest and smallest of the three region areas.}
\CSMeta{\textbf{Ground truth:} 7pi for the full question; 13pi is the intermediate outer-annulus area}
\CSLegend
\CSMeta{Same frozen response, gold-answer hint, and Base student reference.}
\CSRule
\CSModel{OPSD}{-0.048977}{negative}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E17D7D}{-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}The}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}between}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{E17D7D}{6}\CSGap%
\CSToken{EFB7B7}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{light}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}gray}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}which}\CSGap%
\CSToken{E79494}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Z}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F1C3C3}{-}\CSGap%
\CSToken{F7DADA}{\textperiodcentered{}The}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}area}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}between}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F9E4E4}{4}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{EEB6B6}{gray}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{F0BFBF}{\textperiodcentered{}which}\CSGap%
\CSToken{F3C9C9}{\textperiodcentered{}is}\CSGap%
\CSToken{F8DEDE}{\textperiodcentered{}Y}\CSGap%
\CSToken{F6D7D7}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{EEB5B5}{-}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}The}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}between}\CSGap%
\CSToken{EBA8A8}{\textperiodcentered{}}\CSGap%
\CSToken{F1C2C2}{0}\CSGap%
\CSToken{F7DADA}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E69393}{\textperiodcentered{}white}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{'s}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}not}\CSGap%
\CSToken{F3CCCC}{\textperiodcentered{}shaded}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{BFDDCB}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{94C6A9}{\textperiodcentered{}referring}\CSGap%
\CSToken{F6D9D9}{\textperiodcentered{}to}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}three}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}as}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}three}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{E38383}{ular}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{?}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Wait}\CSGap%
\CSToken{F2C5C5}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}but}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}there}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}are}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}two}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}ann}\CSGap%
\CSToken{E9A0A0}{ular}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}one}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}circle}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Wait}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}but}\CSGap%
\CSToken{ECABAB}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}says}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}three}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}labeled}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}X}\CSGap%
\CSToken{FAE7E7}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Y}\CSGap%
\CSToken{F7DDDD}{,}\CSGap%
\CSToken{EDAEAE}{\textperiodcentered{}Z}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Maybe}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{most}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}circle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}considered}\CSGap%
\CSToken{7FBB97}{\textperiodcentered{}a}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}region}\CSGap%
\CSToken{E17D7D}{?}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}in}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}As}\CSGap%
\CSToken{FAE9E9}{ym}\CSGap%
\CSToken{F0F1F2}{pt}\CSGap%
\CSToken{E5F1EA}{ote}\CSGap%
\CSToken{E38383}{\textperiodcentered{}code}\CSGap%
\CSToken{F8E0E0}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}it}\CSGap%
\CSToken{E17D7D}{'s}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}white}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}it}\CSGap%
\CSToken{E17D7D}{'s}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}not}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}shaded}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}considering}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}as}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}three}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}parts}\CSGap%
\CSToken{E17D7D}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{most}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}circle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{white}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}middle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{ECADAD}{ulus}\CSGap%
\CSToken{EAA2A2}{\textperiodcentered{}(}\CSGap%
\CSToken{F9E5E5}{gray}\CSGap%
\CSToken{F4CFCF}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}the}\CSGap%
\CSToken{ECACAC}{\textperiodcentered{}outer}\CSGap%
\CSToken{E38484}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE9E9}{ulus}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F7DDDD}{light}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}gray}\CSGap%
\CSToken{E89C9C}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}says}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}"}\CSGap%
\CSToken{E17D7D}{three}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}are}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}labeled}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}X}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Y}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E68F8F}{\textperiodcentered{}or}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Z}\CSGap%
\CSToken{E58D8D}{\textperiodcentered{}below}\CSGap%
\CSToken{E17D7D}{."}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}So}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{F1C1C1}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}white}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}circle}\CSGap%
\CSToken{F2C6C6}{\textperiodcentered{}is}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}one}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}region}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}middle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{F8E1E1}{ulus}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{EEB5B5}{\textperiodcentered{}another}\CSGap%
\CSToken{ECADAD}{,}\CSGap%
\CSToken{F3CACA}{\textperiodcentered{}and}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}the}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}outer}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE9E9}{ulus}\CSGap%
\CSToken{EEB5B5}{\textperiodcentered{}is}\CSGap%
\CSToken{E69090}{\textperiodcentered{}the}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}third}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}in}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}case}\CSGap%
\CSToken{F9E5E5}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}says}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}"}\CSGap%
\CSToken{E17D7D}{the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}region}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}with}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}the}\CSGap%
\CSToken{F6D9D9}{\textperiodcentered{}greatest}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{"}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}"}\CSGap%
\CSToken{E38282}{the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}region}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}with}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}the}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}smallest}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{."}\CSGap%
\CSToken{A4CFB6}{\textperiodcentered{}The}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}greatest}\CSGap%
\CSToken{E89A9A}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}be}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}outer}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{F9E5E5}{ulus}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{between}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F7DBDB}{6}\CSGap%
\CSToken{E79696}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}smallest}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}be}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{most}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}circle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{radius}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{E17D7D}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}let}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}check}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{62AC80}{Wait}\CSGap%
\CSToken{F3C8C8}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}area}\CSGap%
\CSToken{ECACAC}{\textperiodcentered{}of}\CSGap%
\CSToken{F3CACA}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}outer}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE9E9}{ulus}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{between}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F5D2D2}{6}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{E38585}{)}\CSGap%
\CSToken{EFB9B9}{\textperiodcentered{}is}\CSGap%
\CSToken{E28080}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{E17D7D}{(}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{F6D5D5}{\textsuperscript{2}}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}-}\CSGap%
\CSToken{F6D7D7}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{\textsuperscript{2}}\CSGap%
\CSToken{FAE8E8}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F7DEDE}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F8E2E2}{(}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE8E8}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{EAA3A3}{.\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{F4CFCF}{The}\CSGap%
\CSToken{ECAAAA}{\textperiodcentered{}middle}\CSGap%
\CSToken{F6D6D6}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE7E7}{ulus}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{F6D7D7}{between}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE8E8}{4}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{F7DCDC}{)}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}is}\CSGap%
\CSToken{F4CFCF}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{FAE8E8}{(}\CSGap%
\CSToken{FAE7E7}{6}\CSGap%
\CSToken{FAE9E9}{\textsuperscript{2}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{\textsuperscript{2}}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE8E8}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F9E6E6}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{ECABAB}{The}\CSGap%
\CSToken{F5D3D3}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{most}\CSGap%
\CSToken{F1C4C4}{\textperiodcentered{}circle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{EBA9A9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{E99F9F}{(}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F8E1E1}{\textsuperscript{2}}\CSGap%
\CSToken{F7DEDE}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{E89B9B}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{62AC80}{Wait}\CSGap%
\CSToken{EAA1A1}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}areas}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}are}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{EDB1B1}{1}\CSGap%
\CSToken{E17D7D}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F8DEDE}{2}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}So}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}be}\CSGap%
\CSToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{-}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}The}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}outer}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE7E7}{ulus}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{Z}\CSGap%
\CSToken{E17D7D}{):}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{-}\CSGap%
\CSToken{A5CFB6}{\textperiodcentered{}The}\CSGap%
\CSToken{F7DDDD}{\textperiodcentered{}middle}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE9E9}{ulus}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}(}\CSGap%
\CSToken{F8E1E1}{Y}\CSGap%
\CSToken{FAE8E8}{):}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F8DFDF}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSModel{DCSD}{+0.035223}{positive}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{F6D6D6}{-}\CSGap%
\CSToken{C8E2D2}{\textperiodcentered{}The}\CSGap%
\CSToken{C6E0D1}{\textperiodcentered{}area}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}between}\CSGap%
\CSToken{78B792}{\textperiodcentered{}}\CSGap%
\CSToken{62AC80}{6}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}and}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}(}\CSGap%
\CSToken{DCECE3}{light}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}gray}\CSGap%
\CSToken{E38484}{),}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}which}\CSGap%
\CSToken{E3F0E9}{\textperiodcentered{}is}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Z}\CSGap%
\CSToken{9CCAAE}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E5F1EA}{-}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}The}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}area}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}between}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}and}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{DEEDE4}{\textperiodcentered{}(}\CSGap%
\CSToken{E5F1EA}{gray}\CSGap%
\CSToken{E3F0E8}{),}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}which}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}is}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}Y}\CSGap%
\CSToken{E5F1EA}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E5F1EA}{-}\CSGap%
\CSToken{B4D7C2}{\textperiodcentered{}The}\CSGap%
\CSToken{95C7A9}{\textperiodcentered{}area}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}between}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{0}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}and}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}is}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}white}\CSGap%
\CSToken{DCEDE3}{,}\CSGap%
\CSToken{68AF85}{\textperiodcentered{}so}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{DBECE2}{'s}\CSGap%
\CSToken{E3F0E8}{\textperiodcentered{}not}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}shaded}\CSGap%
\CSToken{CFE6D8}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}the}\CSGap%
\CSToken{D5E8DD}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}referring}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}to}\CSGap%
\CSToken{9FCCB1}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}three}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}regions}\CSGap%
\CSToken{67AE84}{\textperiodcentered{}as}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{DAEBE1}{\textperiodcentered{}three}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}ann}\CSGap%
\CSToken{F0BDBD}{ular}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{?}\CSGap%
\CSToken{DDEDE3}{\textperiodcentered{}Wait}\CSGap%
\CSToken{FAE7E7}{,}\CSGap%
\CSToken{EEB3B3}{\textperiodcentered{}but}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}there}\CSGap%
\CSToken{DAECE1}{\textperiodcentered{}are}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}two}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE8E8}{ular}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}regions}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}one}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}inner}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}circle}\CSGap%
\CSToken{DFEEE5}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Wait}\CSGap%
\CSToken{F5D4D4}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}but}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{CDE4D6}{\textperiodcentered{}problem}\CSGap%
\CSToken{F7DADA}{\textperiodcentered{}says}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}three}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}regions}\CSGap%
\CSToken{F4CDCD}{\textperiodcentered{}labeled}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}X}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}Y}\CSGap%
\CSToken{E4F1E9}{,}\CSGap%
\CSToken{A4CFB6}{\textperiodcentered{}Z}\CSGap%
\CSToken{DDEDE3}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Maybe}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}inner}\CSGap%
\CSToken{62AC80}{most}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}circle}\CSGap%
\CSToken{EDB2B2}{\textperiodcentered{}is}\CSGap%
\CSToken{EBA9A9}{\textperiodcentered{}considered}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}a}\CSGap%
\CSToken{E2F0E8}{\textperiodcentered{}region}\CSGap%
\CSToken{E17D7D}{?}\CSGap%
\CSToken{C1DECD}{\textperiodcentered{}But}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}in}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}the}\CSGap%
\CSToken{BBDBC8}{\textperiodcentered{}As}\CSGap%
\CSToken{FAE9E9}{ym}\CSGap%
\CSToken{E5F1EA}{pt}\CSGap%
\CSToken{E5F1EA}{ote}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}code}\CSGap%
\CSToken{E4F0E9}{,}\CSGap%
\CSToken{F5D1D1}{\textperiodcentered{}it}\CSGap%
\CSToken{C3DFCE}{'s}\CSGap%
\CSToken{D9EBE0}{\textperiodcentered{}white}\CSGap%
\CSToken{E58C8C}{,}\CSGap%
\CSToken{AED4BD}{\textperiodcentered{}so}\CSGap%
\CSToken{EEB5B5}{\textperiodcentered{}maybe}\CSGap%
\CSToken{C7E1D2}{\textperiodcentered{}it}\CSGap%
\CSToken{E3F0E8}{'s}\CSGap%
\CSToken{E0EFE6}{\textperiodcentered{}not}\CSGap%
\CSToken{F7DEDE}{\textperiodcentered{}shaded}\CSGap%
\CSToken{B9DAC7}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}considering}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}regions}\CSGap%
\CSToken{E0EFE6}{\textperiodcentered{}as}\CSGap%
\CSToken{F2C5C5}{\textperiodcentered{}the}\CSGap%
\CSToken{A7D0B8}{\textperiodcentered{}three}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}parts}\CSGap%
\CSToken{62AC80}{:}\CSGap%
\CSToken{C6E1D1}{\textperiodcentered{}the}\CSGap%
\CSToken{DFEEE5}{\textperiodcentered{}inner}\CSGap%
\CSToken{E79595}{most}\CSGap%
\CSToken{EDAFAF}{\textperiodcentered{}circle}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}(}\CSGap%
\CSToken{F6D5D5}{white}\CSGap%
\CSToken{F8E1E1}{),}\CSGap%
\CSToken{E0EFE6}{\textperiodcentered{}the}\CSGap%
\CSToken{E3F0E8}{\textperiodcentered{}middle}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}ann}\CSGap%
\CSToken{E4F1E9}{ulus}\CSGap%
\CSToken{DEEDE4}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{gray}\CSGap%
\CSToken{E5F1EA}{),}\CSGap%
\CSToken{E4F0E9}{\textperiodcentered{}and}\CSGap%
\CSToken{E4F0E9}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}outer}\CSGap%
\CSToken{D9EBE1}{\textperiodcentered{}ann}\CSGap%
\CSToken{F0F1F2}{ulus}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}(}\CSGap%
\CSToken{E5F1EA}{light}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}gray}\CSGap%
\CSToken{D6E9DD}{).}\CSGap%
\CSToken{A3CEB4}{\textperiodcentered{}But}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}problem}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}says}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}"}\CSGap%
\CSToken{CCE4D6}{three}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}regions}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}are}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}labeled}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}X}\CSGap%
\CSToken{E5F1EA}{,}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}Y}\CSGap%
\CSToken{FAE7E7}{,}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}or}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}Z}\CSGap%
\CSToken{DBECE2}{\textperiodcentered{}below}\CSGap%
\CSToken{F5D1D1}{."}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}So}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{F4CECE}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}white}\CSGap%
\CSToken{63AC81}{\textperiodcentered{}inner}\CSGap%
\CSToken{DAEBE1}{\textperiodcentered{}circle}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}is}\CSGap%
\CSToken{E69292}{\textperiodcentered{}one}\CSGap%
\CSToken{B4D7C2}{\textperiodcentered{}region}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}middle}\CSGap%
\CSToken{CFE6D8}{\textperiodcentered{}ann}\CSGap%
\CSToken{E5F1EA}{ulus}\CSGap%
\CSToken{F8DEDE}{\textperiodcentered{}is}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}another}\CSGap%
\CSToken{E5F1EA}{,}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}and}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}outer}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}ann}\CSGap%
\CSToken{F0F1F2}{ulus}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}is}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}third}\CSGap%
\CSToken{62AC80}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}in}\CSGap%
\CSToken{7EBA96}{\textperiodcentered{}that}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}case}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{AFD4BE}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}problem}\CSGap%
\CSToken{94C6A9}{\textperiodcentered{}says}\CSGap%
\CSToken{E58D8D}{\textperiodcentered{}"}\CSGap%
\CSToken{F9E5E5}{the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}region}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}with}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}greatest}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}area}\CSGap%
\CSToken{62AC80}{"}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}and}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}"}\CSGap%
\CSToken{F2C6C6}{the}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}region}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}with}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}the}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}smallest}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}area}\CSGap%
\CSToken{E17D7D}{."}\CSGap%
\CSToken{BBDBC8}{\textperiodcentered{}The}\CSGap%
\CSToken{F7DEDE}{\textperiodcentered{}greatest}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}area}\CSGap%
\CSToken{CCE4D6}{\textperiodcentered{}would}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}be}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}outer}\CSGap%
\CSToken{C7E1D2}{\textperiodcentered{}ann}\CSGap%
\CSToken{E5F1EA}{ulus}\CSGap%
\CSToken{7CB995}{\textperiodcentered{}(}\CSGap%
\CSToken{E3F0E8}{between}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{6}\CSGap%
\CSToken{E3F0E8}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{ADD3BC}{),}\CSGap%
\CSToken{EDAEAE}{\textperiodcentered{}and}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}smallest}\CSGap%
\CSToken{EDAFAF}{\textperiodcentered{}area}\CSGap%
\CSToken{D2E7DB}{\textperiodcentered{}would}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}be}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}the}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}inner}\CSGap%
\CSToken{E17D7D}{most}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}circle}\CSGap%
\CSToken{DFEEE5}{\textperiodcentered{}(}\CSGap%
\CSToken{E5F1EA}{radius}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E4F1E9}{).}\CSGap%
\CSToken{C2DECD}{\textperiodcentered{}But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}let}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}me}\CSGap%
\CSToken{BBDBC8}{\textperiodcentered{}check}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{62AC80}{Wait}\CSGap%
\CSToken{F9E6E6}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}area}\CSGap%
\CSToken{E0EEE6}{\textperiodcentered{}of}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}the}\CSGap%
\CSToken{70B38B}{\textperiodcentered{}outer}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}ann}\CSGap%
\CSToken{FAE9E9}{ulus}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{between}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{6}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{C5E0D0}{)}\CSGap%
\CSToken{CEE5D7}{\textperiodcentered{}is}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{85BE9C}{(}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{E4F1E9}{\textsuperscript{2}}\CSGap%
\CSToken{97C7AA}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\textsuperscript{2}}\CSGap%
\CSToken{E5F1EA}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{E5F1EA}{(}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{C0DECC}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E4F1E9}{The}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}middle}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}ann}\CSGap%
\CSToken{E5F1EA}{ulus}\CSGap%
\CSToken{D2E7DB}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{between}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}and}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{E5F1EA}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}is}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\textsuperscript{2}}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}-}\CSGap%
\CSToken{F7DBDB}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{\textsuperscript{2}}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E4F1E9}{The}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}inner}\CSGap%
\CSToken{B9DAC6}{most}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}circle}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E5F1EA}{\textsuperscript{2}}\CSGap%
\CSToken{E5F1EA}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Wait}\CSGap%
\CSToken{E5F1EA}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{7AB893}{\textperiodcentered{}the}\CSGap%
\CSToken{C8E2D3}{\textperiodcentered{}areas}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}are}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{1}\CSGap%
\CSToken{C2DECD}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{F2C4C4}{,}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{2}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{DCECE3}{\textperiodcentered{}and}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{C7E1D2}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}So}\CSGap%
\CSToken{BFDDCB}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}regions}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}would}\CSGap%
\CSToken{89C09F}{\textperiodcentered{}be}\CSGap%
\CSToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{-}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}The}\CSGap%
\CSToken{A8D1B8}{\textperiodcentered{}outer}\CSGap%
\CSToken{91C4A6}{\textperiodcentered{}ann}\CSGap%
\CSToken{E5F1EA}{ulus}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}(}\CSGap%
\CSToken{B2D6C1}{Z}\CSGap%
\CSToken{E17D7D}{):}\CSGap%
\CSToken{E2EFE7}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{FAE9E9}{\ensuremath{\pi}}\CSGap%
\CSToken{62AC80}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E4F1E9}{-}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}The}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}middle}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}ann}\CSGap%
\CSToken{E5F1EA}{ulus}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}(}\CSGap%
\CSToken{F0F1F2}{Y}\CSGap%
\CSToken{FAE9E9}{):}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{\ensuremath{\pi}}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSMeta{\textbf{The boxed calculation is correct: pi(7\textasciicircum{}2 - 6\textasciicircum{}2) = 13pi. OPSD gives negative mean credit; DCSD gives positive mean credit.}}
\CSMeta{Signal = model(+gold) log-probability minus the same Base(no-answer) log-probability. Colors encode the signal, not mathematical correctness.}
\CSSource{math500\_0279\_s3; context tokens [812, 1231); boxed tokens [1080, 1123). Selected local case, not an overall performance estimate.}
\endgroup


==> case_04.tex <==
% Generated from immutable V2 scored JSON. Native text, not an image.
\begingroup
\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt}
\CSCaseTitle{Case 4: a correct winning move receives opposite credit}
\CSMeta{\textbf{Question:} Alice moves first. Players remove 1 or 4 tokens, and taking the last token wins. Count positive n <= 2024 for which Bob can force a win.}
\CSMeta{\textbf{Ground truth:} 809 for the full question}
\CSLegend
\CSMeta{Same frozen response, gold-answer hint, and Base student reference.}
\CSRule
\CSModel{OPSD}{-0.042883}{negative}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E17D7D}{n}\CSGap%
\CSToken{FAE9E9}{=}\CSGap%
\CSToken{F9E5E5}{4}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}Alice}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}take}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F7DADA}{4}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}win}\CSGap%
\CSToken{A0CCB2}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}So}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE8E8}{4}\CSGap%
\CSToken{E99F9F}{)=}\CSGap%
\CSToken{FAE7E7}{false}\CSGap%
\CSToken{F9E6E6}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F6D9D9}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Alice}\CSGap%
\CSToken{ECADAD}{\textperiodcentered{}can}\CSGap%
\CSToken{F6D7D7}{\textperiodcentered{}take}\CSGap%
\CSToken{F5D2D2}{\textperiodcentered{}}\CSGap%
\CSToken{F9E4E4}{1}\CSGap%
\CSToken{62AC80}{,}\CSGap%
\CSToken{F4D0D0}{\textperiodcentered{}leaving}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F2C6C6}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{L}\CSGap%
\CSToken{ECAAAA}{(}\CSGap%
\CSToken{F9E5E5}{4}\CSGap%
\CSToken{F8E2E2}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}or}\CSGap%
\CSToken{ECABAB}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F6D7D7}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}(}\CSGap%
\CSToken{F8E1E1}{L}\CSGap%
\CSToken{F9E6E6}{(}\CSGap%
\CSToken{FAE8E8}{1}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE8E8}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F9E6E6}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}no}\CSGap%
\CSToken{F4D0D0}{\textperiodcentered{}matter}\CSGap%
\CSToken{F3CBCB}{\textperiodcentered{}what}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}does}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{E89898}{\textperiodcentered{}Bob}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{E69393}{\textperiodcentered{}win}\CSGap%
\CSToken{E69393}{.}\CSGap%
\CSToken{F7DADA}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{EAA2A2}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{ECABAB}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{F9E7E7}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F0BBBB}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE8E8}{6}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F3C9C9}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F6D7D7}{\textperiodcentered{}can}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F8DFDF}{1}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}leaving}\CSGap%
\CSToken{EAA5A5}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}(}\CSGap%
\CSToken{E89999}{L}\CSGap%
\CSToken{EBA8A8}{(}\CSGap%
\CSToken{FAE8E8}{5}\CSGap%
\CSToken{FAE8E8}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{E17D7D}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F8DFDF}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F7DBDB}{\textperiodcentered{}can}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}move}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}to}\CSGap%
\CSToken{ECAAAA}{\textperiodcentered{}a}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}losing}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}position}\CSGap%
\CSToken{C4E0CF}{\textperiodcentered{}for}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Bob}\CSGap%
\CSToken{86BF9D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{F7DBDB}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{F9E5E5}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{F8E0E0}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E79797}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F2C6C6}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}(}\CSGap%
\CSToken{ECACAC}{L}\CSGap%
\CSToken{EFBBBB}{(}\CSGap%
\CSToken{FAE8E8}{6}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}or}\CSGap%
\CSToken{F1C3C3}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F8E1E1}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE8E8}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}no}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}matter}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}what}\CSGap%
\CSToken{E0EEE6}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}does}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{F4CFCF}{\textperiodcentered{}Bob}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}win}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{F4CFCF}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F7DBDB}{,}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{FAE8E8}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{FAE8E8}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E89898}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F5D1D1}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE7E7}{1}\CSGap%
\CSToken{EAA4A4}{,}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F3CCCC}{L}\CSGap%
\CSToken{EDAEAE}{(}\CSGap%
\CSToken{FAE8E8}{7}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{E17D7D}{).}\CSGap%
\CSToken{EEB4B4}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F9E7E7}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F3CCCC}{\textperiodcentered{}can}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}win}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}So}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{F4CDCD}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F6D9D9}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{E17D7D}{4}\CSGap%
\CSToken{EEB3B3}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}(}\CSGap%
\CSToken{F7DEDE}{L}\CSGap%
\CSToken{F7DEDE}{(}\CSGap%
\CSToken{FAE9E9}{5}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{E99F9F}{).}\CSGap%
\CSToken{F6D6D6}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE8E8}{)=}\CSGap%
\CSToken{F9E6E6}{false}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E17D7D}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{E58C8C}{\textperiodcentered{}Alice}\CSGap%
\CSToken{EEB6B6}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}}\CSGap%
\CSToken{F9E6E6}{1}\CSGap%
\CSToken{E38282}{,}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}(}\CSGap%
\CSToken{F1C1C1}{L}\CSGap%
\CSToken{F3CBCB}{(}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{EAA1A1}{\textperiodcentered{}or}\CSGap%
\CSToken{F3CACA}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F9E3E3}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{E58E8E}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}no}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}matter}\CSGap%
\CSToken{F4CECE}{\textperiodcentered{}what}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}does}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}Bob}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}win}\CSGap%
\CSToken{EEB6B6}{.}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F8E1E1}{,}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{BDDCC9}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F8DEDE}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F2C7C7}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F9E4E4}{1}\CSGap%
\CSToken{F4CECE}{,}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F5D3D3}{L}\CSGap%
\CSToken{F1C3C3}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{0}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{E17D7D}{).}\CSGap%
\CSToken{EFB9B9}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE8E8}{false}\CSGap%
\CSToken{F5D4D4}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F1C3C3}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{:}\CSGap%
\CSToken{F7DDDD}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F3C9C9}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F8E0E0}{1}\CSGap%
\CSToken{F6D9D9}{,}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F3CACA}{L}\CSGap%
\CSToken{F2C4C4}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}or}\CSGap%
\CSToken{F4D0D0}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{F9E5E5}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE8E8}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{8}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{E79696}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{F8DFDF}{)=}\CSGap%
\CSToken{F7DADA}{true}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSModel{DCSD}{+0.038157}{positive}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{96C7AA}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{E5F1EA}{4}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Alice}\CSGap%
\CSToken{E58E8E}{\textperiodcentered{}can}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{4}\CSGap%
\CSToken{EFBABA}{\textperiodcentered{}and}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}win}\CSGap%
\CSToken{62AC80}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}So}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{E5F1EA}{4}\CSGap%
\CSToken{E9A0A0}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E5F1EA}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{E58D8D}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{A7D0B8}{,}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}leaving}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}(}\CSGap%
\CSToken{E99F9F}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{E5F1EA}{4}\CSGap%
\CSToken{F9E5E5}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}or}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F8E2E2}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{L}\CSGap%
\CSToken{E5F1EA}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{84BD9B}{\textperiodcentered{}no}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}matter}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}what}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}does}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}Bob}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}win}\CSGap%
\CSToken{DEEEE4}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F8DFDF}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{EEB2B2}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E5F1EA}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{6}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F2C5C5}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F7DCDC}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{F8DFDF}{).}\CSGap%
\CSToken{EAA1A1}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{C0DDCC}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}can}\CSGap%
\CSToken{EDB0B0}{\textperiodcentered{}move}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}to}\CSGap%
\CSToken{DEEDE4}{\textperiodcentered{}a}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}losing}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}position}\CSGap%
\CSToken{F4D1D1}{\textperiodcentered{}for}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}Bob}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}so}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F9E7E7}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E5F1EA}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E4F1E9}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{FAE9E9}{7}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{E69090}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}(}\CSGap%
\CSToken{F0BDBD}{L}\CSGap%
\CSToken{FAE8E8}{(}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}or}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F9E5E5}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{EAA2A2}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}no}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}matter}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}what}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}does}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Bob}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}can}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}win}\CSGap%
\CSToken{DEEDE4}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F9E7E7}{,}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{FAE8E8}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E2F0E8}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE7E7}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F7DADA}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{7}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{F2C7C7}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E48888}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}can}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}win}\CSGap%
\CSToken{9DCBB0}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}So}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{FAE9E9}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}can}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{62AC80}{4}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F9E5E5}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{5}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{F8E1E1}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}L}\CSGap%
\CSToken{E5F1EA}{(}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E5F1EA}{.\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E5F1EA}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE7E7}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F6D9D9}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E27E7E}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}or}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{6}\CSGap%
\CSToken{F0F1F2}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{EDB1B1}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{A2CEB4}{\textperiodcentered{}no}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}matter}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}what}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}does}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Bob}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}win}\CSGap%
\CSToken{FAE9E9}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Alice}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{0}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}(}\CSGap%
\CSToken{F7DCDC}{L}\CSGap%
\CSToken{FAE7E7}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{E5F1EA}{0}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{F4D0D0}{).}\CSGap%
\CSToken{E48888}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{C6E1D1}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{FAE7E7}{n}\CSGap%
\CSToken{F0F1F2}{=}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{:}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}Alice}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}can}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}(}\CSGap%
\CSToken{F8DFDF}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{E89A9A}{),}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}or}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}take}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}leaving}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}(}\CSGap%
\CSToken{FAE9E9}{L}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{8}\CSGap%
\CSToken{F0F1F2}{)=}\CSGap%
\CSToken{FAE9E9}{false}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{F1C2C2}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}L}\CSGap%
\CSToken{F0F1F2}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{FAE9E9}{)=}\CSGap%
\CSToken{FAE9E9}{true}\CSGap%
\CSToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSMeta{\textbf{The boxed move is correct: from 9, remove 4 and leave the opponent losing state 5. Thus L(9)=false. OPSD gives negative mean credit; DCSD gives positive mean credit.}}
\CSMeta{Signal = model(+gold) log-probability minus the same Base(no-answer) log-probability. Colors encode the signal, not mathematical correctness.}
\CSSource{aime24\_0008\_s2; context tokens [4034, 4399); boxed tokens [4235, 4263). Selected local case, not an overall performance estimate.}
\endgroup


==> case_05.tex <==
% Generated from immutable V2 scored JSON. Native text, not an image.
\begingroup
\setlength{\parindent}{0pt}
\setlength{\parskip}{0pt}
\CSCaseTitle{Case 5: a correct remainder calculation receives opposite credit}
\CSMeta{\textbf{Question:} Find the sum of all positive integers n such that n + 2 divides 3(n + 3)(n\textasciicircum{}2 + 9).}
\CSMeta{\textbf{Ground truth:} 49 for the full question; 39 is the intermediate value P(-2)}
\CSLegend
\CSMeta{Same frozen response, gold-answer hint, and Base student reference.}
\CSRule
\CSModel{OPSD}{-0.021065}{negative}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E17D7D}{To}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}approach}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}this}\CSGap%
\CSToken{E38484}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}I}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}can}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}perform}\CSGap%
\CSToken{F5D3D3}{\textperiodcentered{}polynomial}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}division}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}or}\CSGap%
\CSToken{68AF84}{\textperiodcentered{}use}\CSGap%
\CSToken{F1C0C0}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}concept}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}of}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divis}\CSGap%
\CSToken{FAE9E9}{ibility}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Alternatively}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}I}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}use}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}remainder}\CSGap%
\CSToken{F9E2E2}{\textperiodcentered{}theorem}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Let}\CSGap%
\CSToken{F4D0D0}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}think}\CSGap%
\CSToken{62AC80}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{If}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}I}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}consider}\CSGap%
\CSToken{ACD3BC}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}polynomial}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{F6D6D6}{(n}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F4CECE}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{)(}\CSGap%
\CSToken{FAE9E9}{n}\CSGap%
\CSToken{FAE9E9}{\textsuperscript{2}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}and}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}I}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}want}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}to}\CSGap%
\CSToken{F1C3C3}{\textperiodcentered{}divide}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{62AC80}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Then}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}by}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}remainder}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}theorem}\CSGap%
\CSToken{F9E7E7}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}if}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}we}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divide}\CSGap%
\CSToken{F1C1C1}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}by}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}n}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}the}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}remainder}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}should}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}be}\CSGap%
\CSToken{F3CCCC}{\textperiodcentered{}zero}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}So}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}substit}\CSGap%
\CSToken{FAE9E9}{uting}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{F9E7E7}{\textperiodcentered{}into}\CSGap%
\CSToken{E9A0A0}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{F4D0D0}{)}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}should}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}give}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}zero}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Wait}\CSGap%
\CSToken{FAE8E8}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}but}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}be}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}if}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}divides}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{E17D7D}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}However}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}since}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{F3CACA}{\textperiodcentered{}a}\CSGap%
\CSToken{F7DBDB}{\textperiodcentered{}positive}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}integer}\CSGap%
\CSToken{F6D9D9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}definitely}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}not}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}zero}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}but}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}maybe}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}this}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}substitution}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{E27F7F}{\textperiodcentered{}help}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}find}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}some}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}constraints}\CSGap%
\CSToken{E17D7D}{?\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{88C09F}{Let}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}try}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{EBA8A8}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Let}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}me}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}compute}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE7E7}{(-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{):\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{ECACAC}{P}\CSGap%
\CSToken{FAE8E8}{(-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{F0BDBD}{(-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{F2C8C8}{)((}\CSGap%
\CSToken{F5D1D1}{-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{F5D4D4}{)\textasciicircum{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{F8E0E0}{)}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{F9E6E6}{(}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{)(}\CSGap%
\CSToken{FAE9E9}{4}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{C9E2D3}{\textperiodcentered{}*}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F9E3E3}{1}\CSGap%
\CSToken{F2C6C6}{\textperiodcentered{}*}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE8E8}{9}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{E17D7D}{But}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}if}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}n}\CSGap%
\CSToken{F4CDCD}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{F6D9D9}{\textperiodcentered{}divides}\CSGap%
\CSToken{E69191}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{F7DDDD}{\textperiodcentered{}then}\CSGap%
\CSToken{EBA9A9}{\textperiodcentered{}the}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}remainder}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}when}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE8E8}{(n}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}divided}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}by}\CSGap%
\CSToken{F1C3C3}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}zero}\CSGap%
\CSToken{D6E9DE}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}However}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}according}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{F6D7D7}{\textperiodcentered{}the}\CSGap%
\CSToken{E79898}{\textperiodcentered{}remainder}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}theorem}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{F8E0E0}{\textperiodcentered{}remainder}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{)}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE8E8}{9}\CSGap%
\CSToken{F2C4C4}{.}\CSGap%
\CSToken{9DCBAF}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}this}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}suggests}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}}\CSGap%
\CSToken{F9E5E5}{3}\CSGap%
\CSToken{E17D7D}{9}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}must}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}be}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}congr}\CSGap%
\CSToken{FAE9E9}{uent}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}to}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}zero}\CSGap%
\CSToken{F1C0C0}{\textperiodcentered{}modulo}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{ECABAB}{.}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{E89B9B}{,}\CSGap%
\CSToken{E58B8B}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divides}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{E17D7D}{Wait}\CSGap%
\CSToken{EFB9B9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}seems}\CSGap%
\CSToken{F9E3E3}{\textperiodcentered{}like}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}a}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}key}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}insight}\CSGap%
\CSToken{81BC99}{!}\CSGap%
\CSToken{68AF84}{\textperiodcentered{}Because}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}if}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}n}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{F1C3C3}{\textperiodcentered{}divides}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{F7DBDB}{(n}\CSGap%
\CSToken{E17D7D}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}then}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}remainder}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}when}\CSGap%
\CSToken{E38484}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE8E8}{(n}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}divided}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}by}\CSGap%
\CSToken{EDB1B1}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}zero}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}which}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}equal}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}to}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{62AC80}{).}\CSGap%
\CSToken{EEB5B5}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F9E5E5}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divides}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{)}\CSGap%
\CSToken{F6D8D8}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{F9E6E6}{9}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{F1C1C1}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}must}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}be}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}a}\CSGap%
\CSToken{F2C6C6}{\textperiodcentered{}positive}\CSGap%
\CSToken{E27F7F}{\textperiodcentered{}divisor}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}of}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{E17D7D}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Since}\CSGap%
\CSToken{F6D5D5}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}is}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}a}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}positive}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}integer}\CSGap%
\CSToken{FAE7E7}{,}\CSGap%
\CSToken{F2C7C7}{\textperiodcentered{}n}\CSGap%
\CSToken{F4D1D1}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}at}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}least}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}}\CSGap%
\CSToken{E79494}{3}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}(}\CSGap%
\CSToken{E17D7D}{since}\CSGap%
\CSToken{E58F8F}{\textperiodcentered{}n}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}\ensuremath{\geq}}\CSGap%
\CSToken{EEB2B2}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{1}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{E69393}{\textperiodcentered{}n}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}}\CSGap%
\CSToken{FAE8E8}{2}\CSGap%
\CSToken{ECAAAA}{\textperiodcentered{}\ensuremath{\geq}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F3C9C9}{3}\CSGap%
\CSToken{ECACAC}{).}\CSGap%
\CSToken{73B48D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}div}\CSGap%
\CSToken{FAE9E9}{isors}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}of}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{3}\CSGap%
\CSToken{FAE9E9}{9}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{FAE7E7}{\textperiodcentered{}are}\CSGap%
\CSToken{B7D9C5}{\textperiodcentered{}greater}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}than}\CSGap%
\CSToken{F4D0D0}{\textperiodcentered{}or}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}equal}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}to}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F9E6E6}{3}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}are}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E27E7E}{\textperiodcentered{}possible}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}values}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}of}\CSGap%
\CSToken{F1C1C1}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{FAE9E9}{2}\CSGap%
\CSToken{62AC80}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSModel{DCSD}{+0.012545}{positive}
\begingroup\CSTokenFont
\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax
\noindent%
\CSToken{E17D7D}{To}\CSGap%
\CSToken{F8E2E2}{\textperiodcentered{}approach}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}this}\CSGap%
\CSToken{E2EFE7}{,}\CSGap%
\CSToken{9DCBAF}{\textperiodcentered{}maybe}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}I}\CSGap%
\CSToken{F9E5E5}{\textperiodcentered{}can}\CSGap%
\CSToken{D9EBE0}{\textperiodcentered{}perform}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}polynomial}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}division}\CSGap%
\CSToken{E2EFE7}{\textperiodcentered{}or}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}use}\CSGap%
\CSToken{E69191}{\textperiodcentered{}the}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}concept}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}of}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}divis}\CSGap%
\CSToken{F0F1F2}{ibility}\CSGap%
\CSToken{D7EADF}{.}\CSGap%
\CSToken{F4CFCF}{\textperiodcentered{}Alternatively}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}I}\CSGap%
\CSToken{DFEEE5}{\textperiodcentered{}can}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}use}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}remainder}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}theorem}\CSGap%
\CSToken{62AC80}{.}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Let}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}me}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}think}\CSGap%
\CSToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{93C5A7}{If}\CSGap%
\CSToken{D0E6D9}{\textperiodcentered{}I}\CSGap%
\CSToken{D5E9DD}{\textperiodcentered{}consider}\CSGap%
\CSToken{CDE4D6}{\textperiodcentered{}the}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}polynomial}\CSGap%
\CSToken{CAE3D4}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(n}\CSGap%
\CSToken{F0F1F2}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{)(}\CSGap%
\CSToken{F0F1F2}{n}\CSGap%
\CSToken{F0F1F2}{\textsuperscript{2}}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{DAEBE1}{),}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}and}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}I}\CSGap%
\CSToken{E2F0E8}{\textperiodcentered{}want}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}to}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}divide}\CSGap%
\CSToken{E48888}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{EDB0B0}{).}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Then}\CSGap%
\CSToken{E1EFE7}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}by}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}remainder}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}theorem}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{F1C3C3}{\textperiodcentered{}if}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}we}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divide}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{F0F1F2}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}by}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}n}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}the}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}remainder}\CSGap%
\CSToken{C9E2D3}{\textperiodcentered{}should}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}be}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}zero}\CSGap%
\CSToken{E4F1E9}{.}\CSGap%
\CSToken{A1CDB2}{\textperiodcentered{}So}\CSGap%
\CSToken{F6D9D9}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}substit}\CSGap%
\CSToken{F0F1F2}{uting}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}into}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{E4F1E9}{)}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}should}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}give}\CSGap%
\CSToken{B1D6C0}{\textperiodcentered{}zero}\CSGap%
\CSToken{9ECCB1}{.}\CSGap%
\CSToken{F6D9D9}{\textperiodcentered{}Wait}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}but}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}would}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}be}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}if}\CSGap%
\CSToken{A9D1B9}{\textperiodcentered{}n}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divides}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{B5D8C3}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}However}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{E38484}{\textperiodcentered{}since}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{E1EFE7}{\textperiodcentered{}is}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}a}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}positive}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}integer}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{B6D8C4}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F7DBDB}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}definitely}\CSGap%
\CSToken{9DCBAF}{\textperiodcentered{}not}\CSGap%
\CSToken{CBE3D5}{\textperiodcentered{}zero}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}but}\CSGap%
\CSToken{8CC2A1}{\textperiodcentered{}maybe}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}this}\CSGap%
\CSToken{E48888}{\textperiodcentered{}substitution}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}can}\CSGap%
\CSToken{E0EEE6}{\textperiodcentered{}help}\CSGap%
\CSToken{E89999}{\textperiodcentered{}me}\CSGap%
\CSToken{D6E9DE}{\textperiodcentered{}find}\CSGap%
\CSToken{F3CACA}{\textperiodcentered{}some}\CSGap%
\CSToken{EDB1B1}{\textperiodcentered{}constraints}\CSGap%
\CSToken{E17D7D}{?\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{62AC80}{Let}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}me}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}try}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}that}\CSGap%
\CSToken{FAE8E8}{.}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}Let}\CSGap%
\CSToken{F1C2C2}{\textperiodcentered{}me}\CSGap%
\CSToken{EBA8A8}{\textperiodcentered{}compute}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}P}\CSGap%
\CSToken{FAE9E9}{(-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E89A9A}{):\textbackslash{}n\textbackslash{}n}\CSGap%
\CSFocus{%
\CSToken{FAE9E9}{P}\CSGap%
\CSToken{F0F1F2}{(-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{FAE7E7}{(-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F9E2E2}{)((}\CSGap%
\CSToken{E5F1EA}{-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{62AC80}{)\textasciicircum{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{FAE9E9}{)}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{FAE9E9}{(}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{)(}\CSGap%
\CSToken{F0F1F2}{4}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{F0F1F2}{)}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{E58E8E}{\textperiodcentered{}*}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{1}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}*}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{E5F1EA}{9}\CSGap%
\CSToken{62AC80}{.}\CSGap%
\CSToken{D8EADF}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
}%
\noindent%
\CSToken{62AC80}{But}\CSGap%
\CSToken{ECABAB}{\textperiodcentered{}if}\CSGap%
\CSToken{E4F1E9}{\textperiodcentered{}n}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}divides}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{E5F1EA}{),}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}then}\CSGap%
\CSToken{C4E0CF}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}remainder}\CSGap%
\CSToken{DBECE2}{\textperiodcentered{}when}\CSGap%
\CSToken{6AB086}{\textperiodcentered{}P}\CSGap%
\CSToken{E5F1EA}{(n}\CSGap%
\CSToken{F0F1F2}{)}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}is}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}divided}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}by}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{D8EADF}{\textperiodcentered{}is}\CSGap%
\CSToken{D2E7DA}{\textperiodcentered{}zero}\CSGap%
\CSToken{98C8AB}{.}\CSGap%
\CSToken{F5D4D4}{\textperiodcentered{}However}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}according}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}the}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}remainder}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}theorem}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}remainder}\CSGap%
\CSToken{BCDBC9}{\textperiodcentered{}is}\CSGap%
\CSToken{E3F0E8}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E27E7E}{)}\CSGap%
\CSToken{E89A9A}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{DDEDE3}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}this}\CSGap%
\CSToken{AAD2BA}{\textperiodcentered{}suggests}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}that}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{3}\CSGap%
\CSToken{E5F1EA}{9}\CSGap%
\CSToken{D0E6D9}{\textperiodcentered{}must}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}be}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}congr}\CSGap%
\CSToken{F0F1F2}{uent}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}zero}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}modulo}\CSGap%
\CSToken{ECADAD}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{B4D7C3}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{E3F0E8}{,}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divides}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{93C5A7}{.}\CSGap%
\CSToken{C6E1D1}{\textperiodcentered{}\textbackslash{}n\textbackslash{}n}\CSGap%
\CSToken{F0BCBC}{Wait}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}that}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}seems}\CSGap%
\CSToken{D7EADF}{\textperiodcentered{}like}\CSGap%
\CSToken{DEEDE4}{\textperiodcentered{}a}\CSGap%
\CSToken{A9D1B9}{\textperiodcentered{}key}\CSGap%
\CSToken{F8E1E1}{\textperiodcentered{}insight}\CSGap%
\CSToken{E17D7D}{!}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}Because}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}if}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}divides}\CSGap%
\CSToken{D6E9DE}{\textperiodcentered{}P}\CSGap%
\CSToken{E5F1EA}{(n}\CSGap%
\CSToken{C8E2D2}{),}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}then}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}the}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}remainder}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}when}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(n}\CSGap%
\CSToken{F0F1F2}{)}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}is}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}divided}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}by}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F7DCDC}{\textperiodcentered{}is}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}zero}\CSGap%
\CSToken{E17D7D}{,}\CSGap%
\CSToken{76B690}{\textperiodcentered{}which}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}equal}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{DEEDE4}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{62AC80}{).}\CSGap%
\CSToken{F5D1D1}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{FAE9E9}{,}\CSGap%
\CSToken{CAE3D4}{\textperiodcentered{}n}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}divides}\CSGap%
\CSToken{C1DECD}{\textperiodcentered{}P}\CSGap%
\CSToken{F0F1F2}{(-}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{F9E4E4}{)}\CSGap%
\CSToken{F8DFDF}{\textperiodcentered{}=}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{E0EFE6}{.}\CSGap%
\CSToken{E79494}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}must}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}be}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}a}\CSGap%
\CSToken{FAE8E8}{\textperiodcentered{}positive}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}divisor}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}of}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{9CCBAF}{.}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Since}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}is}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}a}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}positive}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}integer}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{E2EFE7}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}is}\CSGap%
\CSToken{89C09F}{\textperiodcentered{}at}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}least}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{E4F1E9}{3}\CSGap%
\CSToken{DDEDE3}{\textperiodcentered{}(}\CSGap%
\CSToken{F1C2C2}{since}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}n}\CSGap%
\CSToken{8EC3A3}{\textperiodcentered{}\ensuremath{\geq}}\CSGap%
\CSToken{F9E4E4}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{1}\CSGap%
\CSToken{D6E9DE}{,}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}so}\CSGap%
\CSToken{E2F0E8}{\textperiodcentered{}n}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}+}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{2}\CSGap%
\CSToken{F9E6E6}{\textperiodcentered{}\ensuremath{\geq}}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}}\CSGap%
\CSToken{E5F1EA}{3}\CSGap%
\CSToken{FAE9E9}{).}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}Therefore}\CSGap%
\CSToken{F0F1F2}{,}\CSGap%
\CSToken{66AE83}{\textperiodcentered{}the}\CSGap%
\CSToken{F2C4C4}{\textperiodcentered{}div}\CSGap%
\CSToken{F0F1F2}{isors}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}of}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{F0F1F2}{9}\CSGap%
\CSToken{9AC9AD}{\textperiodcentered{}that}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}are}\CSGap%
\CSToken{E17D7D}{\textperiodcentered{}greater}\CSGap%
\CSToken{9DCBB0}{\textperiodcentered{}than}\CSGap%
\CSToken{E5F1EA}{\textperiodcentered{}or}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}equal}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}to}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{3}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}are}\CSGap%
\CSToken{D1E6D9}{\textperiodcentered{}the}\CSGap%
\CSToken{62AC80}{\textperiodcentered{}possible}\CSGap%
\CSToken{E99F9F}{\textperiodcentered{}values}\CSGap%
\CSToken{F2C6C6}{\textperiodcentered{}of}\CSGap%
\CSToken{FAE9E9}{\textperiodcentered{}n}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}+}\CSGap%
\CSToken{F0F1F2}{\textperiodcentered{}}\CSGap%
\CSToken{F0F1F2}{2}\CSGap%
\CSToken{E69393}{.\textbackslash{}n\textbackslash{}n}\CSGap%
\par\endgroup
\CSRule
\CSMeta{\textbf{The boxed calculation is correct: P(-2) = 3(-2 + 3)((-2)\textasciicircum{}2 + 9) = 39. OPSD gives negative mean credit; DCSD gives positive mean credit.}}
\CSMeta{Signal = model(+gold) log-probability minus the same Base(no-answer) log-probability. Colors encode the signal, not mathematical correctness.}
\CSSource{aime25\_0016\_s3; context tokens [201, 626); boxed tokens [363, 411). Selected local case, not an overall performance estimate.}
\endgroup


==> case_study_macros.tex <==
% Load this file ONCE in the preamble. No tabularx, TikZ, or PythonTeX.
\RequirePackage{xcolor}
\RequirePackage{textcomp}
\definecolor{CSInk}{HTML}{202629}
\definecolor{CSGray}{HTML}{586368}
\definecolor{CSRuleColor}{HTML}{DAE0E1}
\definecolor{CSPositive}{RGB}{54,148,92}
\definecolor{CSNegative}{RGB}{217,88,88}
\newcommand{\CSTokenFont}{\fontsize{7.5}{10.5}\selectfont\ttfamily\color{CSInk}}
\newcommand{\CSToken}[2]{{\setlength{\fboxsep}{0.45pt}\colorbox[HTML]{#1}{\rule[-1.875pt]{0pt}{7.5pt}#2}}}
\newcommand{\CSGap}{\hskip 0.55pt plus .15pt minus .1pt\relax}
\newsavebox{\CSFocusMeasure}
\newcommand{\CSFocus}[1]{%
  \par\vspace{3pt}\noindent
  \begingroup\setlength{\fboxsep}{2pt}\setlength{\fboxrule}{0.65pt}%
  \sbox{\CSFocusMeasure}{#1\unskip}%
  \ifdim\dimexpr\wd\CSFocusMeasure+2\fboxsep+2\fboxrule\relax>\linewidth
    \fbox{\begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}%
      \CSTokenFont\rightskip=0pt plus 1fil\parfillskip=0pt\noindent#1\unskip\par
    \end{minipage}}%
  \else
    \fbox{\usebox{\CSFocusMeasure}}%
  \fi
  \endgroup\par\vspace{3pt}\noindent\ignorespaces
}
\newcommand{\CSCaseTitle}[1]{\par{\color{CSInk}\sffamily\bfseries\fontsize{13}{15}\selectfont #1\par}\vspace{6pt}}
\newcommand{\CSMeta}[1]{\par{\color{CSInk}\sffamily\fontsize{8.5}{10.5}\selectfont #1\par}\vspace{3pt}}
\newcommand{\CSSource}[1]{\par{\color{CSGray}\sffamily\fontsize{7}{8.5}\selectfont #1\par}}
\newcommand{\CSRule}{\par\vspace{6pt}{\color{CSRuleColor}\hrule height .4pt}\vspace{5pt}}
\newcommand{\CSModel}[3]{\par{\sffamily\color{CSInk}\bfseries\fontsize{10}{12}\selectfont #1\hfill
  {\normalfont\sffamily\fontsize{8}{10}\selectfont Boxed span mean: #2 nat/token (#3)}\par}\nobreak\vspace{4pt}}
\newcommand{\CSLegend}{\CSMeta{%
  \textcolor{CSPositive}{\rule{5pt}{5pt}} Positive\quad
  \textcolor{CSNegative}{\rule{5pt}{5pt}} Negative\quad
  Black frame: selected span. Shared color saturation: 0.1 nat.}}


==> prompt_horizontal/all_prompt_cases_horizontal.tex <==
\input{prompt_horizontal/prompt_case_01_horizontal.tex}
\par\vspace{6pt}
\input{prompt_horizontal/prompt_case_02_horizontal.tex}
\par\vspace{6pt}
\input{prompt_horizontal/prompt_case_03_horizontal.tex}
\par\vspace{6pt}
\input{prompt_horizontal/prompt_case_04_horizontal.tex}
\par\vspace{6pt}
\input{prompt_horizontal/prompt_case_05_horizontal.tex}
\par\vspace{6pt}


==> prompt_horizontal/prompt_case_01_horizontal.tex <==
% Flowing side-by-side LaTeX. Each model row stays intact; the whole case may break.
\par\begingroup
\setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\PHInit
\PHTitle{A. Correct factorization \textbar{} token-level evidence}
\PHMeta{\textbf{Question:} Let \(p(x)\) be a polynomial of degree 5 such that \(p(n) = \frac{n}{n^2 - 1}\)for \(n = 2,\) 3, 4, \(\dots,\) 7.  Find \(p(8).\)}
\PHMeta{\textbf{Gold:} \(\frac{3}{56}\)\quad math500\_0011\_s2; paragraph 74}
\PHMeta{P1/P3: identical answer information and words; the reference-answer block moves before the question.}
\PHLegend
\vspace{5pt}
\PHRow{}{\PHColumnTitle{P1: reference after question}}{\PHColumnTitle{P3: reference before question}}
\nobreak\vspace{4pt}
\PHRow{Base}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{DDEDE4}{Then}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{B7D9C5}{.}\PHGap%
\PHToken{E38383}{\textperiodcentered{}So}\PHGap%
\PHToken{F7DDDD}{,}\PHGap%
\PHToken{EBA9A9}{\textperiodcentered{}total}\PHGap%
\PHToken{DEEEE4}{\textperiodcentered{}is}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{D2E7DA}{/}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{E2EFE7}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE7E7}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F4CDCD}{To}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}combine}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}these}\PHGap%
\PHToken{EDAEAE}{\textperiodcentered{}fractions}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{DEEEE5}{\textperiodcentered{}find}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}a}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}common}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E5F1EA}{.}\PHGap%
\PHToken{D9EBE0}{\textperiodcentered{}Let}\PHGap%
\PHToken{F6D9D9}{'s}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}see}\PHGap%
\PHToken{F8E0E0}{,}\PHGap%
\PHToken{C6E1D1}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{8BC1A1}{.}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}Let}\PHGap%
\PHToken{CDE4D6}{\textperiodcentered{}me}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}find}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{E17D7D}{(}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{C6E1D1}{).}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Prime}\PHGap%
\PHToken{DCECE3}{\textperiodcentered{}factors}\PHGap%
\PHToken{F1C2C2}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E4F1E9}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{94C6A8}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E17D7D}{2}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F4D0D0}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{B9DAC6}{6}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE7E7}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{62AC80}{So}\PHGap%
\PHToken{DBECE2}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{F8DEDE}{\textperiodcentered{}is}\PHGap%
\PHToken{F6D8D8}{\textperiodcentered{}max}\PHGap%
\PHToken{E0EFE6}{\textperiodcentered{}ex}\PHGap%
\PHToken{F0F1F2}{ponents}\PHGap%
\PHToken{E4F1EA}{:}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{62AC80}{,}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{BCDCC9}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}So}\PHGap%
\PHToken{ADD3BC}{\textperiodcentered{}}\PHGap%
\PHToken{D9EBE0}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{9ECCB1}{\textperiodcentered{}=}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F9E4E4}{*}\PHGap%
\PHToken{F8E0E0}{9}\PHGap%
\PHToken{D6E9DE}{=}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{C6E0D1}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{CFE5D8}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.003166}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{DDEDE4}{Then}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{B8D9C5}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{C9E2D3}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}total}\PHGap%
\PHToken{D4E8DC}{\textperiodcentered{}is}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{D0E6D9}{/}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}-}\PHGap%
\PHToken{F8E1E1}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F8E2E2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F1BFBF}{To}\PHGap%
\PHToken{F7DADA}{\textperiodcentered{}combine}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}these}\PHGap%
\PHToken{E38282}{\textperiodcentered{}fractions}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}find}\PHGap%
\PHToken{E1EFE7}{\textperiodcentered{}a}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}common}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E5F1EA}{.}\PHGap%
\PHToken{E0EEE6}{\textperiodcentered{}Let}\PHGap%
\PHToken{DEEDE4}{'s}\PHGap%
\PHToken{F8DEDE}{\textperiodcentered{}see}\PHGap%
\PHToken{E2F0E8}{,}\PHGap%
\PHToken{B7D9C5}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{67AE84}{.}\PHGap%
\PHToken{DCECE3}{\textperiodcentered{}Let}\PHGap%
\PHToken{DCECE3}{\textperiodcentered{}me}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}find}\PHGap%
\PHToken{F2C5C5}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{E17D7D}{(}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{C8E1D2}{).}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Prime}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}factors}\PHGap%
\PHToken{F2C7C7}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E4F1E9}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{6CB188}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{D9EBE0}{2}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F2C7C7}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{C2DFCE}{6}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F9E5E5}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{62AC80}{So}\PHGap%
\PHToken{DEEDE4}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{F6D9D9}{\textperiodcentered{}is}\PHGap%
\PHToken{EEB5B5}{\textperiodcentered{}max}\PHGap%
\PHToken{E1EFE6}{\textperiodcentered{}ex}\PHGap%
\PHToken{F0F1F2}{ponents}\PHGap%
\PHToken{E5F1EA}{:}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{62AC80}{,}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{C8E1D2}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}So}\PHGap%
\PHToken{9AC9AD}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{F4CFCF}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F8E0E0}{*}\PHGap%
\PHToken{F6D6D6}{9}\PHGap%
\PHToken{D5E9DD}{=}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{BFDDCB}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{CDE4D6}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.003356}}{+}
}%
\PHRule
\PHRow{OPSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E17D7D}{Then}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{E27F7F}{3}\PHGap%
\PHToken{FAE9E9}{/}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}total}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}is}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E17D7D}{/}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{)}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE8E8}{/}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{To}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}combine}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}these}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}fractions}\PHGap%
\PHToken{F9E4E4}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}find}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}a}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}common}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F4D0D0}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Let}\PHGap%
\PHToken{F7DBDB}{'s}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}see}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{E9A0A0}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{F2C6C6}{\textperiodcentered{}and}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Let}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}me}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}find}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}L}\PHGap%
\PHToken{FAE9E9}{CM}\PHGap%
\PHToken{62AC80}{(}\PHGap%
\PHToken{F8DFDF}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{).}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Prime}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}factors}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{EBA8A8}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{8CC2A2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{62AC80}{2}\PHGap%
\PHToken{F8E1E1}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE7E7}{3}\PHGap%
\PHToken{FAE8E8}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F1C2C2}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{F3C9C9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}}\PHGap%
\PHToken{E17D7D}{2}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{E17D7D}{6}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE7E7}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{So}\PHGap%
\PHToken{E48A8A}{\textperiodcentered{}L}\PHGap%
\PHToken{FAE9E9}{CM}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}is}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}max}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}ex}\PHGap%
\PHToken{FAE9E9}{ponents}\PHGap%
\PHToken{E17D7D}{:}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{CEE5D7}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F7DADA}{3}\PHGap%
\PHToken{FAE8E8}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{F5D4D4}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{E17D7D}{6}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{F4CFCF}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{F9E5E5}{6}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{*}\PHGap%
\PHToken{E17D7D}{9}\PHGap%
\PHToken{E17D7D}{=}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}}\PHGap%
\PHToken{FAE8E8}{5}\PHGap%
\PHToken{F5D4D4}{7}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F0BEBE}{5}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{C7E1D2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.000635}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E17D7D}{Then}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{E48787}{3}\PHGap%
\PHToken{FAE9E9}{/}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}total}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}is}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E17D7D}{/}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{)}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE8E8}{/}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{To}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}combine}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}these}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}fractions}\PHGap%
\PHToken{F9E4E4}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}find}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}a}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}common}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F5D2D2}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Let}\PHGap%
\PHToken{FAE7E7}{'s}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}see}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{EAA1A1}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{F3C9C9}{\textperiodcentered{}and}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Let}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}me}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}find}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}L}\PHGap%
\PHToken{FAE9E9}{CM}\PHGap%
\PHToken{62AC80}{(}\PHGap%
\PHToken{F8DFDF}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{E17D7D}{).}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Prime}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}factors}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{ECABAB}{5}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{78B792}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{62AC80}{2}\PHGap%
\PHToken{F8E2E2}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE7E7}{3}\PHGap%
\PHToken{FAE8E8}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F3C9C9}{4}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{F4CECE}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{E17D7D}{2}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{E17D7D}{6}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE8E8}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E27F7F}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{So}\PHGap%
\PHToken{E48989}{\textperiodcentered{}L}\PHGap%
\PHToken{FAE9E9}{CM}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}is}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}max}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}ex}\PHGap%
\PHToken{FAE9E9}{ponents}\PHGap%
\PHToken{E17D7D}{:}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{E4F1E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F7DCDC}{3}\PHGap%
\PHToken{FAE8E8}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{F5D3D3}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{E17D7D}{6}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{F3CBCB}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{F9E6E6}{6}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{*}\PHGap%
\PHToken{E17D7D}{9}\PHGap%
\PHToken{E17D7D}{=}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}}\PHGap%
\PHToken{FAE8E8}{5}\PHGap%
\PHToken{F6D6D6}{7}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F1C2C2}{5}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{ACD3BC}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.000579}}{+}
}%
\PHRule
\PHRow{DCSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{D8EAE0}{Then}\PHGap%
\PHToken{FAE7E7}{,}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{64AC81}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{D7EADF}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}total}\PHGap%
\PHToken{DDEDE4}{\textperiodcentered{}is}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{BDDCCA}{/}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{E4F0E9}{)}\PHGap%
\PHToken{DEEEE5}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F6D7D7}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{To}\PHGap%
\PHToken{F1C0C0}{\textperiodcentered{}combine}\PHGap%
\PHToken{F6D5D5}{\textperiodcentered{}these}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}fractions}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{C8E2D3}{\textperiodcentered{}find}\PHGap%
\PHToken{CDE5D7}{\textperiodcentered{}a}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}common}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E5F1EA}{.}\PHGap%
\PHToken{D4E8DC}{\textperiodcentered{}Let}\PHGap%
\PHToken{A5CFB6}{'s}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}see}\PHGap%
\PHToken{F0BBBB}{,}\PHGap%
\PHToken{6EB289}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{62AC80}{.}\PHGap%
\PHToken{D1E6DA}{\textperiodcentered{}Let}\PHGap%
\PHToken{E4F0E9}{\textperiodcentered{}me}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}find}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{E17D7D}{(}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{85BE9C}{).}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Prime}\PHGap%
\PHToken{CEE5D8}{\textperiodcentered{}factors}\PHGap%
\PHToken{FAE8E8}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E4F0E9}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{90C4A5}{2}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E89999}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E4F1E9}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E4F1E9}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{62AC80}{6}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F8E0E0}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{62AC80}{So}\PHGap%
\PHToken{CCE4D5}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{F6D6D6}{\textperiodcentered{}is}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}max}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}ex}\PHGap%
\PHToken{F0F1F2}{ponents}\PHGap%
\PHToken{E2F0E8}{:}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{62AC80}{,}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{E4F1E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E48888}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}So}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}}\PHGap%
\PHToken{B3D6C1}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{E1EFE7}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{E68F8F}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{DEEEE4}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F1C2C2}{*}\PHGap%
\PHToken{E89898}{9}\PHGap%
\PHToken{C5E0D0}{=}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{90C4A5}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{C3DFCE}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.009834}}{+}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{D8EADF}{Then}\PHGap%
\PHToken{FAE7E7}{,}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{66AE83}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{AFD4BE}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}total}\PHGap%
\PHToken{CDE4D6}{\textperiodcentered{}is}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{BCDBC8}{/}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{E3F0E9}{)}\PHGap%
\PHToken{DFEEE5}{\textperiodcentered{}-}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{/}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F5D2D2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{To}\PHGap%
\PHToken{EDAEAE}{\textperiodcentered{}combine}\PHGap%
\PHToken{F4D0D0}{\textperiodcentered{}these}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}fractions}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{C6E0D0}{\textperiodcentered{}find}\PHGap%
\PHToken{C7E1D2}{\textperiodcentered{}a}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}common}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E5F1EA}{.}\PHGap%
\PHToken{D6E9DE}{\textperiodcentered{}Let}\PHGap%
\PHToken{78B792}{'s}\PHGap%
\PHToken{F8E0E0}{\textperiodcentered{}see}\PHGap%
\PHToken{F2C7C7}{,}\PHGap%
\PHToken{65AD82}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{62AC80}{.}\PHGap%
\PHToken{D3E7DB}{\textperiodcentered{}Let}\PHGap%
\PHToken{F3CACA}{\textperiodcentered{}me}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}find}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{E17D7D}{(}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{F8E0E0}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{8DC2A2}{).}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Prime}\PHGap%
\PHToken{CDE5D7}{\textperiodcentered{}factors}\PHGap%
\PHToken{D0E6D9}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E4F0E9}{5}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{62AC80}{2}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E48888}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E4F1E9}{4}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{E2F0E8}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E4F1E9}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{63AC81}{6}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F7DDDD}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{62AC80}{So}\PHGap%
\PHToken{D0E6D9}{\textperiodcentered{}L}\PHGap%
\PHToken{F0F1F2}{CM}\PHGap%
\PHToken{F4D1D1}{\textperiodcentered{}is}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}max}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}ex}\PHGap%
\PHToken{F0F1F2}{ponents}\PHGap%
\PHToken{E2F0E8}{:}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{62AC80}{,}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{E4F1E9}{,}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}So}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}}\PHGap%
\PHToken{B8D9C5}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{E2EFE7}{\textperiodcentered{}*}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{F8DEDE}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}*}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}=}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{EEB4B4}{*}\PHGap%
\PHToken{E69292}{9}\PHGap%
\PHToken{C5E0D0}{=}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{77B791}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{BEDCCA}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.014129}}{+}
}%
\par\noindent\begin{minipage}{\linewidth}
\PHRule
\PHMeta{\textbf{Interpretation:} The boxed factorization is correct. Base and OPSD cross zero; DCSD stays positive. OPSD's change is small and close to zero. The adjacent 4480 factorization is incorrect but still receives positive DCSD mean credit.}
\PHMeta{Signal = model(gold prompt) logp - the same Base(no-answer) logp. Colors encode relative support, not correctness. Mean is for the black frame only.}
\PHSource{Context tokens [2497, 2686); selected tokens [2575, 2596). Selected local example, not an overall ranking.}
\end{minipage}\par\endgroup


==> prompt_horizontal/prompt_case_02_horizontal.tex <==
% Flowing side-by-side LaTeX. Each model row stays intact; the whole case may break.
\par\begingroup
\setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\PHInit
\PHTitle{B. Formatting separator \textbar{} token-level evidence}
\PHMeta{\textbf{Question:} Let \(\triangle ABC\) have circumcenter \(O\) and incenter \(I\) with \(\overline{IA}\perp\overline{OI}\), circumradius \(13\), and inradius \(6\). Find \(AB\cdot AC\).}
\PHMeta{\textbf{Gold:} \(468\)\quad aime24\_0016\_s3; paragraph 107}
\PHMeta{P1/P3: identical answer information and words; the reference-answer block moves before the question.}
\PHLegend
\vspace{5pt}
\PHRow{}{\PHColumnTitle{P1: reference after question}}{\PHColumnTitle{P3: reference before question}}
\nobreak\vspace{4pt}
\PHRow{Base}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{FAE9E9}{Now}\PHGap%
\PHToken{FAE8E8}{,}\PHGap%
\PHToken{CFE6D8}{\textperiodcentered{}use}\PHGap%
\PHToken{E4F0E9}{\textperiodcentered{}the}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}identity}\PHGap%
\PHToken{FAE7E7}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F9E3E3}{cos}\PHGap%
\PHToken{E69393}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{FAE9E9}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE8E8}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE7E7}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{E5F1EA}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE9E9}{)\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E0EFE6}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{E4F1EA}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE8E8}{3}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F7DADA}{frac}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{sqrt}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{FAE8E8}{3}\PHGap%
\PHToken{E5F1EA}{0}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE7E7}{---\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{A2CEB4}{\textperiodcentered{}Use}\PHGap%
\PHToken{C7E1D2}{\textperiodcentered{}the}\PHGap%
\PHToken{BFDDCB}{\textperiodcentered{}Law}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}of}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}Cos}\PHGap%
\PHToken{E5F1EA}{ines}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}to}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}Find}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{CDE5D7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F9E6E6}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F9E5E5}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{E5F1EA}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{DDEDE3}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E4F1E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{C3DFCF}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{7CB995}{9}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E5F1EA}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F4CFCF}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{7}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.002246}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{F4CFCF}{Now}\PHGap%
\PHToken{D2E7DA}{,}\PHGap%
\PHToken{BDDCC9}{\textperiodcentered{}use}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{F6D9D9}{\textperiodcentered{}identity}\PHGap%
\PHToken{F9E4E4}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F9E5E5}{cos}\PHGap%
\PHToken{E17D7D}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{FAE9E9}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE8E8}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E6E6}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{E5F1EA}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE9E9}{)\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE8E8}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E7E7}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE8E8}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE8E8}{3}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{C7E1D1}{frac}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{sqrt}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F9E5E5}{3}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{\}\}}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{E5F1EA}{\}\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{C1DECC}{---\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E5F1EA}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{A6D0B7}{\textperiodcentered{}Use}\PHGap%
\PHToken{CBE3D5}{\textperiodcentered{}the}\PHGap%
\PHToken{F5D4D4}{\textperiodcentered{}Law}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}of}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Cos}\PHGap%
\PHToken{E5F1EA}{ines}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}to}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}Find}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}\$\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{BADAC7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F9E4E4}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sin}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{E4F1E9}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{DEEDE4}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{ACD3BC}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{62AC80}{9}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E5F1EA}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F4CDCD}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.027798}}{+}
}%
\PHRule
\PHRow{OPSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E17D7D}{Now}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}use}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}identity}\PHGap%
\PHToken{E0EEE6}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{EBA8A8}{cos}\PHGap%
\PHToken{E17D7D}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{F8E2E2}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F9E4E4}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE7E7}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F5D4D4}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{FAE7E7}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F8DFDF}{)\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{E0EEE6}{\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E17D7D}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F8DFDF}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F8E2E2}{sqrt}\PHGap%
\PHToken{FAE8E8}{\{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E2F0E8}{3}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{6BB087}{frac}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{F2C6C6}{---\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Use}\PHGap%
\PHToken{7FBB97}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Law}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}of}\PHGap%
\PHToken{F6D5D5}{\textperiodcentered{}Cos}\PHGap%
\PHToken{FAE8E8}{ines}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}to}\PHGap%
\PHToken{E48888}{\textperiodcentered{}Find}\PHGap%
\PHToken{F6D6D6}{\textperiodcentered{}\$}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E3E3}{cos}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}A}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}\$\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}A}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F3C9C9}{\textperiodcentered{}}\PHGap%
\PHToken{F9E6E6}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{B8D9C6}{\textbackslash{}}\PHGap%
\PHToken{F8E1E1}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{F9E3E3}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F5D3D3}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F3CCCC}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{EBA8A8}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F9E7E7}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{E17D7D}{9}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE8E8}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E79595}{\}}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE8E8}{7}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.032733}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E17D7D}{Now}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}use}\PHGap%
\PHToken{F5D3D3}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}identity}\PHGap%
\PHToken{F7DDDD}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{EAA4A4}{cos}\PHGap%
\PHToken{E17D7D}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{F9E2E2}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F9E4E4}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{F9E7E7}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F5D1D1}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{FAE7E7}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F8DEDE}{)\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{E0EEE6}{\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E17D7D}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F8DFDF}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F8E1E1}{sqrt}\PHGap%
\PHToken{FAE8E8}{\{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E2F0E8}{3}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{62AC80}{frac}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE8E8}{3}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E0EEE5}{---\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Use}\PHGap%
\PHToken{8EC3A3}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Law}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}of}\PHGap%
\PHToken{F5D1D1}{\textperiodcentered{}Cos}\PHGap%
\PHToken{FAE8E8}{ines}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}to}\PHGap%
\PHToken{E58D8D}{\textperiodcentered{}Find}\PHGap%
\PHToken{F6D6D6}{\textperiodcentered{}\$}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E3E3}{cos}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}A}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}\$\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}A}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F2C7C7}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{B4D7C2}{\textbackslash{}}\PHGap%
\PHToken{F8E2E2}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{F9E4E4}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F5D3D3}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F3CACA}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{EAA4A4}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F9E7E7}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{E17D7D}{9}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE8E8}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E89999}{\}}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE8E8}{7}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.004091}}{+}
}%
\PHRule
\PHRow{DCSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{62AC80}{Now}\PHGap%
\PHToken{F7DDDD}{,}\PHGap%
\PHToken{DBECE1}{\textperiodcentered{}use}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}the}\PHGap%
\PHToken{E0EEE6}{\textperiodcentered{}identity}\PHGap%
\PHToken{FAE7E7}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F7DBDB}{cos}\PHGap%
\PHToken{E17D7D}{\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{left}\PHGap%
\PHToken{FAE7E7}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{F9E7E7}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E4E4}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{FAE9E9}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE8E8}{)\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE8E8}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F8DFDF}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E4F1E9}{3}\PHGap%
\PHToken{E5F1EA}{9}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E6E6}{sqrt}\PHGap%
\PHToken{FAE8E8}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{AFD4BE}{frac}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{sqrt}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F9E5E5}{3}\PHGap%
\PHToken{E5F1EA}{0}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{E5F1EA}{\}\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E17D7D}{---\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E5F1EA}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{8CC2A2}{\textperiodcentered{}Use}\PHGap%
\PHToken{AFD5BE}{\textperiodcentered{}the}\PHGap%
\PHToken{9CCAAF}{\textperiodcentered{}Law}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}of}\PHGap%
\PHToken{F9E7E7}{\textperiodcentered{}Cos}\PHGap%
\PHToken{FAE9E9}{ines}\PHGap%
\PHToken{F2C8C8}{\textperiodcentered{}to}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}Find}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F5D3D3}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F6D7D7}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F6DADA}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{FAE9E9}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE8E8}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{2}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{95C6A9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{62AC80}{9}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E5F1EA}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F5D1D1}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{7}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.132922}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{62AC80}{Now}\PHGap%
\PHToken{DEEEE4}{,}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}use}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}the}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}identity}\PHGap%
\PHToken{F8E1E1}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F8DFDF}{cos}\PHGap%
\PHToken{E17D7D}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{left}\PHGap%
\PHToken{F9E6E6}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE7E7}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F8E2E2}{sin}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{left}\PHGap%
\PHToken{FAE9E9}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE8E8}{)\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sqrt}\PHGap%
\PHToken{FAE7E7}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F6D9D9}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E4F1EA}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F9E5E5}{sqrt}\PHGap%
\PHToken{FAE8E8}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{72B48C}{frac}\PHGap%
\PHToken{FAE9E9}{\{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{sqrt}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F8E2E2}{3}\PHGap%
\PHToken{E5F1EA}{0}\PHGap%
\PHToken{FAE9E9}{\}\}}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{E5F1EA}{\}\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E17D7D}{---\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E5F1EA}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{4}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{8EC3A4}{\textperiodcentered{}Use}\PHGap%
\PHToken{B2D6C0}{\textperiodcentered{}the}\PHGap%
\PHToken{D1E6DA}{\textperiodcentered{}Law}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}of}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}Cos}\PHGap%
\PHToken{E5F1EA}{ines}\PHGap%
\PHToken{F2C6C6}{\textperiodcentered{}to}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}Find}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{cos}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}A}\PHGap%
\PHToken{E4F0E9}{\textperiodcentered{}\$\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F9E2E2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cos}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}A}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F5D3D3}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F7DDDD}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{sin}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{left}\PHGap%
\PHToken{E5F1EA}{(\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{A}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{right}\PHGap%
\PHToken{FAE8E8}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{2}\PHGap%
\PHToken{C7E1D1}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{7FBB97}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{62AC80}{9}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E5F1EA}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F4D0D0}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{frac}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{E5F1EA}{7}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.103710}}{-}
}%
\par\noindent\begin{minipage}{\linewidth}
\PHRule
\PHMeta{\textbf{Interpretation:} The separator adds no mathematical information. Base and OPSD cross zero; DCSD stays negative. A stable negative sign is not a correctness label, and DCSD's magnitude still changes.}
\PHMeta{Signal = model(gold prompt) logp - the same Base(no-answer) logp. Colors encode relative support, not correctness. Mean is for the black frame only.}
\PHSource{Context tokens [5932, 6105); selected tokens [6020, 6021). Selected local example, not an overall ranking.}
\end{minipage}\par\endgroup


==> prompt_horizontal/prompt_case_03_horizontal.tex <==
% Flowing side-by-side LaTeX. Each model row stays intact; the whole case may break.
\par\begingroup
\setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\PHInit
\PHTitle{C. Final-answer heading \textbar{} token-level evidence}
\PHMeta{\textbf{Question:} William Sydney Porter tried to perform the calculation \(\frac{-3+4i}{1+2i}\). However, he accidentally missed the minus sign, finding \(\frac{3+4i}{1+2i}=\frac{11}{5}-\frac{2}{5}i\). What answer should he have obtained?}
\PHMeta{\textbf{Gold:} \(1+2i\)\quad math500\_0373\_s2; paragraph 112}
\PHMeta{P2/P3: identical answer information; both equivalent wording and answer-block position change.}
\PHLegend
\vspace{5pt}
\PHRow{}{\PHColumnTitle{P2: reference after question}}{\PHColumnTitle{P3: reference before question}}
\nobreak\vspace{4pt}
\PHRow{Base}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{DEEDE4}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E38686}{=}\PHGap%
\PHToken{D1E6DA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F8E0E0}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{DDEDE3}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E4F1E9}{)\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F9E3E3}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{8}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{B9D9C6}{\textbackslash{}n}\PHGap%
\PHToken{E2EFE7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{=}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F4CFCF}{)}\PHGap%
\PHToken{ABD2BB}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E2EFE7}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{99C9AC}{\textperiodcentered{}Divide}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}the}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}Result}\PHGap%
\PHToken{CBE3D4}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{D7EADE}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{95C7A9}{\textperiodcentered{}Final}\PHGap%
\PHToken{E79898}{\textperiodcentered{}Answer}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E38282}{The}\PHGap%
\PHToken{D7EADE}{\textperiodcentered{}correct}\PHGap%
\PHToken{F7DEDE}{\textperiodcentered{}result}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}of}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}the}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}calculation}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}is}\PHGap%
\PHToken{FAE8E8}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{boxed}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{62AC80}{<|im\_end|>}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.004014}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E0EFE6}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E58B8B}{=}\PHGap%
\PHToken{CFE6D8}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{C2DECD}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{B9DAC6}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE8E8}{)\textbackslash{}n}\PHGap%
\PHToken{DFEEE5}{\$\$}\PHGap%
\PHToken{F9E4E4}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{8}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{CCE4D5}{\textbackslash{}n}\PHGap%
\PHToken{E2EFE7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F3CCCC}{)}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{DDEDE4}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{8CC2A1}{\textperiodcentered{}Divide}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}the}\PHGap%
\PHToken{C5E0D0}{\textperiodcentered{}Result}\PHGap%
\PHToken{C1DECD}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E1EFE7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E2EFE7}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Final}\PHGap%
\PHToken{80BC98}{\textperiodcentered{}Answer}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F7DCDC}{The}\PHGap%
\PHToken{CCE4D6}{\textperiodcentered{}correct}\PHGap%
\PHToken{E99C9C}{\textperiodcentered{}result}\PHGap%
\PHToken{F3CBCB}{\textperiodcentered{}of}\PHGap%
\PHToken{8AC1A0}{\textperiodcentered{}the}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}calculation}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}is}\PHGap%
\PHToken{FAE9E9}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{boxed}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{62AC80}{<|im\_end|>}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.052538}}{+}
}%
\PHRule
\PHRow{OPSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{F1C2C2}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{EAA2A2}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{F9E2E2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F6D9D9}{\textperiodcentered{}+}\PHGap%
\PHToken{E89B9B}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{E17D7D}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{EFB7B7}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F8E1E1}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{E38484}{)\textbackslash{}n}\PHGap%
\PHToken{F5D5D5}{\$\$}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}-}\PHGap%
\PHToken{F3CACA}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F8E1E1}{i}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F8E0E0}{\textbackslash{}n}\PHGap%
\PHToken{F9E4E4}{\$\$}\PHGap%
\PHToken{EBA5A5}{\textbackslash{}n}\PHGap%
\PHToken{EFB8B8}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{F9E6E6}{=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}}\PHGap%
\PHToken{F9E7E7}{1}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{F2C4C4}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F4CFCF}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E17D7D}{)}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}=}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F2C5C5}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{C8E2D2}{\textperiodcentered{}Divide}\PHGap%
\PHToken{78B792}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Result}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F4CFCF}{\{}\PHGap%
\PHToken{F9E6E6}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F8E2E2}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F2C5C5}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{F7DDDD}{\#\#\#}\PHGap%
\PHToken{F2C4C4}{\textperiodcentered{}Final}\PHGap%
\PHToken{DCEDE3}{\textperiodcentered{}Answer}\PHGap%
\PHToken{F4CFCF}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E17D7D}{The}\PHGap%
\PHToken{E79494}{\textperiodcentered{}correct}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}result}\PHGap%
\PHToken{F9E7E7}{\textperiodcentered{}of}\PHGap%
\PHToken{8DC2A3}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}calculation}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}is}\PHGap%
\PHToken{F3C8C8}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{boxed}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{62AC80}{<|im\_end|>}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.015834}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{F3C9C9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{EDAFAF}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}+}\PHGap%
\PHToken{EBA8A8}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{E17D7D}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F1BFBF}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{E89999}{)\textbackslash{}n}\PHGap%
\PHToken{F8DFDF}{\$\$}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{6}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}-}\PHGap%
\PHToken{F4CFCF}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F9E3E3}{i}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F8E2E2}{\textbackslash{}n}\PHGap%
\PHToken{F9E6E6}{\$\$}\PHGap%
\PHToken{F2C7C7}{\textbackslash{}n}\PHGap%
\PHToken{F2C4C4}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE7E7}{=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}}\PHGap%
\PHToken{FAE8E8}{1}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E48A8A}{\textperiodcentered{}-}\PHGap%
\PHToken{F3C9C9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F5D5D5}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E17D7D}{)}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{0}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{E27F7F}{\textperiodcentered{}=}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F4CECE}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{BDDCC9}{\textperiodcentered{}Divide}\PHGap%
\PHToken{7EBA96}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Result}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F6D6D6}{\{}\PHGap%
\PHToken{FAE7E7}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F9E4E4}{\}}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F4D1D1}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{F8E0E0}{\#\#\#}\PHGap%
\PHToken{A0CCB2}{\textperiodcentered{}Final}\PHGap%
\PHToken{99C9AC}{\textperiodcentered{}Answer}\PHGap%
\PHToken{F6D8D8}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E17D7D}{The}\PHGap%
\PHToken{EDAEAE}{\textperiodcentered{}correct}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}result}\PHGap%
\PHToken{F7DEDE}{\textperiodcentered{}of}\PHGap%
\PHToken{7FBB97}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}calculation}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}is}\PHGap%
\PHToken{F5D1D1}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{boxed}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{62AC80}{<|im\_end|>}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.021468}}{+}
}%
\PHRule
\PHRow{DCSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{CFE6D8}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{=}\PHGap%
\PHToken{D6E9DE}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}+}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{B5D8C3}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E6E6}{)\textbackslash{}n}\PHGap%
\PHToken{DBECE2}{\$\$}\PHGap%
\PHToken{F6D7D7}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{8}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{C2DFCE}{\textbackslash{}n}\PHGap%
\PHToken{E1EFE7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F8E0E0}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F6D5D5}{)}\PHGap%
\PHToken{9CCBAF}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{E2F0E7}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F9E5E5}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Divide}\PHGap%
\PHToken{D8EADF}{\textperiodcentered{}the}\PHGap%
\PHToken{B3D7C2}{\textperiodcentered{}Result}\PHGap%
\PHToken{CAE3D4}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F3CCCC}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{E5F1EA}{\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F7DDDD}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE8E8}{\#\#\#}\PHGap%
\PHToken{9DCBAF}{\textperiodcentered{}Final}\PHGap%
\PHToken{F6D6D6}{\textperiodcentered{}Answer}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{9FCCB1}{The}\PHGap%
\PHToken{D5E8DD}{\textperiodcentered{}correct}\PHGap%
\PHToken{F5D2D2}{\textperiodcentered{}result}\PHGap%
\PHToken{F8E0E0}{\textperiodcentered{}of}\PHGap%
\PHToken{B6D8C4}{\textperiodcentered{}the}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}calculation}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}is}\PHGap%
\PHToken{F8E2E2}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{boxed}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{62AC80}{<|im\_end|>}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.009179}}{+}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{D7EADE}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E27F7F}{=}\PHGap%
\PHToken{D0E6D9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{A7D0B8}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{8DC2A2}{)}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{cdot}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(-}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E5E5}{)\textbackslash{}n}\PHGap%
\PHToken{D5E9DD}{\$\$}\PHGap%
\PHToken{F6D9D9}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{6}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{8}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{D9EBE0}{\textbackslash{}n}\PHGap%
\PHToken{E1EFE7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{=}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{E4F1E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F4D1D1}{)}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E4F1E9}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Divide}\PHGap%
\PHToken{D9EBE1}{\textperiodcentered{}the}\PHGap%
\PHToken{B0D5BF}{\textperiodcentered{}Result}\PHGap%
\PHToken{C1DECD}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F2C7C7}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{E5F1EA}{\{}\PHGap%
\PHToken{E5F1EA}{5}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{0}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{E5F1EA}{\}}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F9E4E4}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE8E8}{\#\#\#}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Final}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}Answer}\PHGap%
\PHToken{E4F0E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{62AC80}{The}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}correct}\PHGap%
\PHToken{E79595}{\textperiodcentered{}result}\PHGap%
\PHToken{F1C1C1}{\textperiodcentered{}of}\PHGap%
\PHToken{72B48D}{\textperiodcentered{}the}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}calculation}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}is}\PHGap%
\PHToken{F9E3E3}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{E5F1EA}{boxed}\PHGap%
\PHToken{F0F1F2}{\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{62AC80}{<|im\_end|>}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.058210}}{+}
}%
\par\noindent\begin{minipage}{\linewidth}
\PHRule
\PHMeta{\textbf{Interpretation:} The heading is stylistic. Base and OPSD cross zero for P2/P3; DCSD stays positive. This does not show absence of a style preference. Base does not flip for P1/P3 here.}
\PHMeta{Signal = model(gold prompt) logp - the same Base(no-answer) logp. Colors encode relative support, not correctness. Mean is for the black frame only.}
\PHSource{Context tokens [3104, 3263); selected tokens [3238, 3242). Selected local example, not an overall ranking.}
\end{minipage}\par\endgroup


==> prompt_horizontal/prompt_case_04_horizontal.tex <==
% Flowing side-by-side LaTeX. Each model row stays intact; the whole case may break.
\par\begingroup
\setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\PHInit
\PHTitle{D. Bezout identity (supplementary) \textbar{} token-level evidence}
\PHMeta{\textbf{Question:} Compute \(17^{-1}\pmod{83}\). Express your answer as a residue from \(0\) to \(82\), inclusive.  (You may find it helpful to consider the fact that \(17\cdot 5=85\).)}
\PHMeta{\textbf{Gold:} \(44\)\quad math500\_0448\_s3; paragraph 19}
\PHMeta{P1/P3: identical answer information and words; the reference-answer block moves before the question.}
\PHLegend
\vspace{5pt}
\PHRow{}{\PHColumnTitle{P1: reference after question}}{\PHColumnTitle{P3: reference before question}}
\nobreak\vspace{4pt}
\PHRow{Base}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{62AC80}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{*(}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{Therefore}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{BCDBC8}{\textperiodcentered{}rearr}\PHGap%
\PHToken{F8DFDF}{anged}\PHGap%
\PHToken{E69090}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{78B791}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F5D2D2}{Which}\PHGap%
\PHToken{EFBBBB}{\textperiodcentered{}means}\PHGap%
\PHToken{E2F0E8}{\textperiodcentered{}that}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E5E5}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E5F1EA}{*}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E38686}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E2F0E7}{.}\PHGap%
\PHToken{F4D0D0}{\textperiodcentered{}Therefore}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}comparing}\PHGap%
\PHToken{A6D0B7}{\textperiodcentered{}to}\PHGap%
\PHToken{E1EFE7}{\textperiodcentered{}the}\PHGap%
\PHToken{CBE4D5}{\textperiodcentered{}equation}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}ax}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}by}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E2F0E7}{\textperiodcentered{}have}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}x}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}y}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{C3DFCF}{.}\PHGap%
\PHToken{F8E1E1}{\textperiodcentered{}However}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{F2C6C6}{\textperiodcentered{}we}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}need}\PHGap%
\PHToken{B8D9C5}{\textperiodcentered{}x}\PHGap%
\PHToken{F0BDBD}{\textperiodcentered{}to}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}be}\PHGap%
\PHToken{D3E7DB}{\textperiodcentered{}a}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}positive}\PHGap%
\PHToken{99C9AC}{\textperiodcentered{}residue}\PHGap%
\PHToken{BCDBC9}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{A5CFB6}{.}\PHGap%
\PHToken{87BF9E}{\textperiodcentered{}So}\PHGap%
\PHToken{DBECE2}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{F5D1D1}{\textperiodcentered{}need}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}to}\PHGap%
\PHToken{F8E1E1}{\textperiodcentered{}find}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}the}\PHGap%
\PHToken{F0BCBC}{\textperiodcentered{}equivalent}\PHGap%
\PHToken{BFDDCB}{\textperiodcentered{}positive}\PHGap%
\PHToken{C4E0CF}{\textperiodcentered{}value}\PHGap%
\PHToken{E0EEE6}{\textperiodcentered{}of}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.005481}}{+}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{62AC80}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{*(}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{Therefore}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{ADD4BD}{\textperiodcentered{}rearr}\PHGap%
\PHToken{F3CCCC}{anged}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E17D7D}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F5D1D1}{Which}\PHGap%
\PHToken{E58C8C}{\textperiodcentered{}means}\PHGap%
\PHToken{E2F0E8}{\textperiodcentered{}that}\PHGap%
\PHToken{E2F0E8}{\textperiodcentered{}-}\PHGap%
\PHToken{E2F0E8}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E5F1EA}{*}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E1EFE7}{.}\PHGap%
\PHToken{EEB4B4}{\textperiodcentered{}Therefore}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}comparing}\PHGap%
\PHToken{A5CFB6}{\textperiodcentered{}to}\PHGap%
\PHToken{C2DFCE}{\textperiodcentered{}the}\PHGap%
\PHToken{C7E1D2}{\textperiodcentered{}equation}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}ax}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}by}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}have}\PHGap%
\PHToken{DEEEE5}{\textperiodcentered{}x}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F6D6D6}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}y}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{CAE3D4}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}However}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{EFB7B7}{\textperiodcentered{}we}\PHGap%
\PHToken{DCEDE3}{\textperiodcentered{}need}\PHGap%
\PHToken{E0EFE6}{\textperiodcentered{}x}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}to}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}be}\PHGap%
\PHToken{66AE83}{\textperiodcentered{}a}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}positive}\PHGap%
\PHToken{A7D0B8}{\textperiodcentered{}residue}\PHGap%
\PHToken{BEDDCB}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{A1CDB3}{.}\PHGap%
\PHToken{72B48C}{\textperiodcentered{}So}\PHGap%
\PHToken{B9DAC6}{,}\PHGap%
\PHToken{E27E7E}{\textperiodcentered{}we}\PHGap%
\PHToken{F7DEDE}{\textperiodcentered{}need}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}to}\PHGap%
\PHToken{DFEEE5}{\textperiodcentered{}find}\PHGap%
\PHToken{B1D6C0}{\textperiodcentered{}the}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}equivalent}\PHGap%
\PHToken{9FCCB1}{\textperiodcentered{}positive}\PHGap%
\PHToken{C3DFCF}{\textperiodcentered{}value}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}of}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.034254}}{-}
}%
\PHRule
\PHRow{OPSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{EDAEAE}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE8E8}{*}\PHGap%
\PHToken{F0BFBF}{3}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{EEB4B4}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F3CBCB}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E58B8B}{*(}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE7E7}{2}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}+}\PHGap%
\PHToken{EFB8B8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F4CECE}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE8E8}{*}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{Therefore}\PHGap%
\PHToken{F7DDDD}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}rearr}\PHGap%
\PHToken{E17D7D}{anged}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{62AC80}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E6E6}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F8E2E2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E17D7D}{Which}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}means}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}that}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E17D7D}{*}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E48888}{\textperiodcentered{}+}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}}\PHGap%
\PHToken{FAE8E8}{8}\PHGap%
\PHToken{E17D7D}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E69292}{\textperiodcentered{}Therefore}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}comparing}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}to}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}equation}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}ax}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E79797}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}have}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}x}\PHGap%
\PHToken{ECAAAA}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E69090}{\textperiodcentered{}and}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}y}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}However}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}need}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}x}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}to}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}be}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}a}\PHGap%
\PHToken{E9A0A0}{\textperiodcentered{}positive}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}residue}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}modulo}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}need}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}to}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}find}\PHGap%
\PHToken{DDEDE3}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}equivalent}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}positive}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}value}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}of}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}modulo}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{F5D3D3}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.003009}}{+}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{EEB6B6}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F5D1D1}{3}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{EFBBBB}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F3C8C8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E69393}{*(}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE8E8}{2}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}+}\PHGap%
\PHToken{EDB0B0}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{F5D2D2}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE8E8}{*}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{Therefore}\PHGap%
\PHToken{F8DFDF}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}rearr}\PHGap%
\PHToken{E17D7D}{anged}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{62AC80}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E6E6}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{F8E1E1}{.\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E17D7D}{Which}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}means}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}that}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E17D7D}{*}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{7}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}+}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{EEB6B6}{3}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E48989}{\textperiodcentered{}Therefore}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}comparing}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}to}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}equation}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}ax}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E89B9B}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}have}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}x}\PHGap%
\PHToken{ECAAAA}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{E69090}{\textperiodcentered{}and}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}y}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}However}\PHGap%
\PHToken{FAE9E9}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}need}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}x}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}to}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}be}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}a}\PHGap%
\PHToken{E48888}{\textperiodcentered{}positive}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}residue}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}modulo}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{E17D7D}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}So}\PHGap%
\PHToken{E17D7D}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}need}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}to}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}find}\PHGap%
\PHToken{EAA4A4}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}equivalent}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}positive}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}value}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}of}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{9}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}modulo}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{8}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{F6D8D8}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.000763}}{-}
}%
\PHRule
\PHRow{DCSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{62AC80}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{*(}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F3C9C9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{Therefore}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{91C5A6}{\textperiodcentered{}rearr}\PHGap%
\PHToken{F4CCCC}{anged}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E17D7D}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F1BFBF}{Which}\PHGap%
\PHToken{E69090}{\textperiodcentered{}means}\PHGap%
\PHToken{E0EEE6}{\textperiodcentered{}that}\PHGap%
\PHToken{E2F0E7}{\textperiodcentered{}-}\PHGap%
\PHToken{DDEDE3}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E5F1EA}{*}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E0EFE6}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Therefore}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}comparing}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}to}\PHGap%
\PHToken{68AE84}{\textperiodcentered{}the}\PHGap%
\PHToken{B7D9C5}{\textperiodcentered{}equation}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}ax}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}by}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{DFEEE5}{\textperiodcentered{}have}\PHGap%
\PHToken{D3E7DB}{\textperiodcentered{}x}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F5D2D2}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}y}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{A7D0B8}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}However}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{EBA7A7}{\textperiodcentered{}we}\PHGap%
\PHToken{DDEDE4}{\textperiodcentered{}need}\PHGap%
\PHToken{78B791}{\textperiodcentered{}x}\PHGap%
\PHToken{E99C9C}{\textperiodcentered{}to}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}be}\PHGap%
\PHToken{C5E0D0}{\textperiodcentered{}a}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}positive}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}residue}\PHGap%
\PHToken{B4D7C3}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{85BE9C}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}So}\PHGap%
\PHToken{62AC80}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{EAA1A1}{\textperiodcentered{}need}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}to}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}find}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}the}\PHGap%
\PHToken{F6D6D6}{\textperiodcentered{}equivalent}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}positive}\PHGap%
\PHToken{BBDBC8}{\textperiodcentered{}value}\PHGap%
\PHToken{DAEBE1}{\textperiodcentered{}of}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.041986}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{E5F1EA}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{62AC80}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F9E3E3}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{*(}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}+}\PHGap%
\PHToken{EAA3A3}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E5F1EA}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{Therefore}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{8CC2A2}{\textperiodcentered{}rearr}\PHGap%
\PHToken{ECADAD}{anged}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E17D7D}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F4CECE}{Which}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}means}\PHGap%
\PHToken{E0EEE6}{\textperiodcentered{}that}\PHGap%
\PHToken{E2EFE7}{\textperiodcentered{}-}\PHGap%
\PHToken{D8EADF}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{FAE9E9}{*}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{7}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{E5F1EA}{3}\PHGap%
\PHToken{F0F1F2}{*}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E0EFE6}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Therefore}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}comparing}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}to}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}the}\PHGap%
\PHToken{B4D7C2}{\textperiodcentered{}equation}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}ax}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}by}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E5F1EA}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{E0EEE6}{\textperiodcentered{}have}\PHGap%
\PHToken{D4E8DC}{\textperiodcentered{}x}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{EFB9B9}{\textperiodcentered{}and}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}y}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{A8D1B9}{.}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}However}\PHGap%
\PHToken{F0F1F2}{,}\PHGap%
\PHToken{E79797}{\textperiodcentered{}we}\PHGap%
\PHToken{CFE6D8}{\textperiodcentered{}need}\PHGap%
\PHToken{87BF9E}{\textperiodcentered{}x}\PHGap%
\PHToken{E1EFE6}{\textperiodcentered{}to}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}be}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}a}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}positive}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}residue}\PHGap%
\PHToken{B6D8C4}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{83BD9B}{.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}So}\PHGap%
\PHToken{62AC80}{,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}we}\PHGap%
\PHToken{F1C0C0}{\textperiodcentered{}need}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}to}\PHGap%
\PHToken{D8EADF}{\textperiodcentered{}find}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}the}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}equivalent}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}positive}\PHGap%
\PHToken{BADAC7}{\textperiodcentered{}value}\PHGap%
\PHToken{E1EFE7}{\textperiodcentered{}of}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{F0F1F2}{9}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}modulo}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{8}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{.\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.122632}}{-}
}%
\par\noindent\begin{minipage}{\linewidth}
\PHRule
\PHMeta{\textbf{Interpretation:} The boxed equality is correct: -17*39 + 83*8 = 1. DCSD stays negative while Base and OPSD cross zero. This is sign stability, NOT evidence that DCSD assigns mathematically correct credit.}
\PHMeta{Signal = model(gold prompt) logp - the same Base(no-answer) logp. Colors encode relative support, not correctness. Mean is for the black frame only.}
\PHSource{Context tokens [661, 811); selected tokens [717, 732). Selected local example, not an overall ranking.}
\end{minipage}\par\endgroup


==> prompt_horizontal/prompt_case_05_horizontal.tex <==
% Flowing side-by-side LaTeX. Each model row stays intact; the whole case may break.
\par\begingroup
\setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\PHInit
\PHTitle{E. Conjugate rationalization (supplementary) \textbar{} token-level evidence}
\PHMeta{\textbf{Question:} William Sydney Porter tried to perform the calculation \(\frac{-3+4i}{1+2i}\). However, he accidentally missed the minus sign, finding \(\frac{3+4i}{1+2i}=\frac{11}{5}-\frac{2}{5}i\). What answer should he have obtained?}
\PHMeta{\textbf{Gold:} \(1+2i\)\quad math500\_0373\_s1; paragraph 69}
\PHMeta{P1/P3: identical answer information and words; the reference-answer block moves before the question.}
\PHLegend
\vspace{5pt}
\PHRow{}{\PHColumnTitle{P1: reference after question}}{\PHColumnTitle{P3: reference before question}}
\nobreak\vspace{4pt}
\PHRow{Base}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{FAE9E9}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{D3E7DB}{\textperiodcentered{}Step}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{D8EAE0}{\textperiodcentered{}Multiply}\PHGap%
\PHToken{E89A9A}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{F2C4C4}{\textperiodcentered{}Con}\PHGap%
\PHToken{FAE9E9}{jug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{F8E1E1}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F7DADA}{The}\PHGap%
\PHToken{6EB28A}{\textperiodcentered{}denominator}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}is}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E2EFE7}{\$,}\PHGap%
\PHToken{F3C8C8}{\textperiodcentered{}so}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}its}\PHGap%
\PHToken{C4E0CF}{\textperiodcentered{}conjug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}is}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E3F0E8}{\$.}\PHGap%
\PHToken{F5D5D5}{\textperiodcentered{}We}\PHGap%
\PHToken{E2EFE7}{\textperiodcentered{}multiply}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}both}\PHGap%
\PHToken{F5D2D2}{\textperiodcentered{}the}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}numerator}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}and}\PHGap%
\PHToken{D0E6D9}{\textperiodcentered{}denominator}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}by}\PHGap%
\PHToken{E2EFE7}{\textperiodcentered{}this}\PHGap%
\PHToken{F4CECE}{\textperiodcentered{}conjug}\PHGap%
\PHToken{E5F1EA}{ate}\PHGap%
\PHToken{E1EFE7}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{EDB2B2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F0F1F2}{(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)\}}\PHGap%
\PHToken{FAE9E9}{\{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{E5F1EA}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{F2C8C8}{\textperiodcentered{}Simpl}\PHGap%
\PHToken{F0F1F2}{ify}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}the}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Den}\PHGap%
\PHToken{F0F1F2}{ominator}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{62AC80}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E5F1EA}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE8E8}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F6D9D9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E58F8F}{i}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F7DBDB}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.001043}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{FAE9E9}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{CFE5D8}{\textperiodcentered{}Step}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{F5D2D2}{\textperiodcentered{}Multiply}\PHGap%
\PHToken{E2F0E8}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{F1C3C3}{\textperiodcentered{}Con}\PHGap%
\PHToken{F0F1F2}{jug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{F9E3E3}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{B5D7C3}{The}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}is}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F8E2E2}{\$,}\PHGap%
\PHToken{EEB5B5}{\textperiodcentered{}so}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}its}\PHGap%
\PHToken{C5E0D0}{\textperiodcentered{}conjug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}is}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E4F1E9}{\$.}\PHGap%
\PHToken{BADBC7}{\textperiodcentered{}We}\PHGap%
\PHToken{E2F0E8}{\textperiodcentered{}multiply}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}both}\PHGap%
\PHToken{F4CDCD}{\textperiodcentered{}the}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}numerator}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}and}\PHGap%
\PHToken{CFE5D8}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E0EFE6}{\textperiodcentered{}by}\PHGap%
\PHToken{DEEDE4}{\textperiodcentered{}this}\PHGap%
\PHToken{F3CBCB}{\textperiodcentered{}conjug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{D9EBE0}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{96C7A9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F0F1F2}{(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)\}}\PHGap%
\PHToken{FAE9E9}{\{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{2}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{F4CECE}{\textperiodcentered{}Simpl}\PHGap%
\PHToken{F0F1F2}{ify}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}Den}\PHGap%
\PHToken{F0F1F2}{ominator}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{99C9AC}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE8E8}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F1C0C0}{i}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F7DCDC}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.001234}}{+}
}%
\PHRule
\PHRow{OPSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{F1C3C3}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{E89C9C}{\textperiodcentered{}Step}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{:}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Multiply}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Con}\PHGap%
\PHToken{FAE9E9}{jug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{The}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F3CCCC}{\textperiodcentered{}is}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE8E8}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{E17D7D}{\$,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}so}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}its}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}conjug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}is}\PHGap%
\PHToken{F3CBCB}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E17D7D}{\$.}\PHGap%
\PHToken{92C5A7}{\textperiodcentered{}We}\PHGap%
\PHToken{E48686}{\textperiodcentered{}multiply}\PHGap%
\PHToken{EFBBBB}{\textperiodcentered{}both}\PHGap%
\PHToken{99C8AC}{\textperiodcentered{}the}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}numerator}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}and}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}by}\PHGap%
\PHToken{F1BFBF}{\textperiodcentered{}this}\PHGap%
\PHToken{E58F8F}{\textperiodcentered{}conjug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE8E8}{\{-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E4E4}{\}}\PHGap%
\PHToken{F3C8C8}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F9E3E3}{\{}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\}}\PHGap%
\PHToken{FAE9E9}{\{(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE8E8}{)\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F2C7C7}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Simpl}\PHGap%
\PHToken{FAE9E9}{ify}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}the}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Den}\PHGap%
\PHToken{FAE9E9}{ominator}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F1C1C1}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F7DBDB}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{)\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F9E4E4}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{i}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{EAA3A3}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F9E5E5}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F7DCDC}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.000915}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{F2C6C6}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{EAA4A4}{\textperiodcentered{}Step}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{:}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Multiply}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}by}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}the}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Con}\PHGap%
\PHToken{FAE9E9}{jug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{E17D7D}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{The}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F3CCCC}{\textperiodcentered{}is}\PHGap%
\PHToken{F7DDDD}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE8E8}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E17D7D}{\$,}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}so}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}its}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}conjug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}is}\PHGap%
\PHToken{F4CFCF}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E17D7D}{\$.}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}We}\PHGap%
\PHToken{E68F8F}{\textperiodcentered{}multiply}\PHGap%
\PHToken{F0BFBF}{\textperiodcentered{}both}\PHGap%
\PHToken{9BCAAE}{\textperiodcentered{}the}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}numerator}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}and}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}by}\PHGap%
\PHToken{F3CBCB}{\textperiodcentered{}this}\PHGap%
\PHToken{E69292}{\textperiodcentered{}conjug}\PHGap%
\PHToken{FAE9E9}{ate}\PHGap%
\PHToken{E17D7D}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE8E8}{\{-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}\{}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E5E5}{\}}\PHGap%
\PHToken{ADD3BD}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{F9E4E4}{\{}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{FAE9E9}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\}}\PHGap%
\PHToken{FAE9E9}{\{(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE8E8}{)\}\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{F4CDCD}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\#\#\#}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}Simpl}\PHGap%
\PHToken{FAE9E9}{ify}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}the}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}Den}\PHGap%
\PHToken{FAE9E9}{ominator}\PHGap%
\PHToken{FAE8E8}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E17D7D}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F8DEDE}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F3CBCB}{\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{F8DFDF}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}(}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{i}\PHGap%
\PHToken{FAE9E9}{)\textasciicircum{}}\PHGap%
\PHToken{FAE9E9}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}-}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{i}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F6D7D7}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}-}\PHGap%
\PHToken{EEB2B2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{)}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{E0EFE6}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F8E2E2}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{5}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n}\PHGap%
\PHToken{FAE9E9}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHPositive}{+0.000625}}{+}
}%
\PHRule
\PHRow{DCSD}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{FAE7E7}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\#\#\#}\PHGap%
\PHToken{C4E0CF}{\textperiodcentered{}Step}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{C8E2D2}{\textperiodcentered{}Multiply}\PHGap%
\PHToken{EEB5B5}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}the}\PHGap%
\PHToken{F4CFCF}{\textperiodcentered{}Con}\PHGap%
\PHToken{FAE9E9}{jug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{F7DBDB}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F2C6C6}{The}\PHGap%
\PHToken{62AC80}{\textperiodcentered{}denominator}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}is}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F9E6E6}{\$,}\PHGap%
\PHToken{E79797}{\textperiodcentered{}so}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}its}\PHGap%
\PHToken{ADD4BD}{\textperiodcentered{}conjug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}is}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}\$}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{DAEBE1}{\$.}\PHGap%
\PHToken{F5D1D1}{\textperiodcentered{}We}\PHGap%
\PHToken{DFEEE5}{\textperiodcentered{}multiply}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}both}\PHGap%
\PHToken{F8E0E0}{\textperiodcentered{}the}\PHGap%
\PHToken{E4F0E9}{\textperiodcentered{}numerator}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}and}\PHGap%
\PHToken{BFDDCB}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F9E6E6}{\textperiodcentered{}by}\PHGap%
\PHToken{CFE5D8}{\textperiodcentered{}this}\PHGap%
\PHToken{F4CDCD}{\textperiodcentered{}conjug}\PHGap%
\PHToken{E5F1EA}{ate}\PHGap%
\PHToken{F9E5E5}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{E17D7D}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F0F1F2}{(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)\}}\PHGap%
\PHToken{FAE9E9}{\{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE9E9}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{EBA6A6}{\textperiodcentered{}Simpl}\PHGap%
\PHToken{F0F1F2}{ify}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}the}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}Den}\PHGap%
\PHToken{F0F1F2}{ominator}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{62AC80}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{E5F1EA}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E5F1EA}{i}\PHGap%
\PHToken{FAE9E9}{)\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F1C0C0}{\textperiodcentered{}}\PHGap%
\PHToken{FAE9E9}{4}\PHGap%
\PHToken{E17D7D}{i}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E4F1E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F3C8C8}{\textperiodcentered{}-}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F1C0C0}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.002488}}{-}
}%
{%
\begingroup\PHTokenFont\rightskip=0pt plus 1fil\relax
\parfillskip=0pt\relax\tolerance=9999\relax\noindent%
\PHToken{F9E6E6}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{\#\#\#}\PHGap%
\PHToken{C2DECD}{\textperiodcentered{}Step}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}Multiply}\PHGap%
\PHToken{C2DECD}{\textperiodcentered{}by}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{F4CECE}{\textperiodcentered{}Con}\PHGap%
\PHToken{FAE9E9}{jug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{F7DCDC}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{C7E1D2}{The}\PHGap%
\PHToken{F0BDBD}{\textperiodcentered{}denominator}\PHGap%
\PHToken{F9E5E5}{\textperiodcentered{}is}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{FAE9E9}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F7DCDC}{\$,}\PHGap%
\PHToken{E27E7E}{\textperiodcentered{}so}\PHGap%
\PHToken{E4F0E9}{\textperiodcentered{}its}\PHGap%
\PHToken{B0D5BF}{\textperiodcentered{}conjug}\PHGap%
\PHToken{F0F1F2}{ate}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}is}\PHGap%
\PHToken{E4F1EA}{\textperiodcentered{}\$}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{DBECE2}{\$.}\PHGap%
\PHToken{BEDCCA}{\textperiodcentered{}We}\PHGap%
\PHToken{DEEDE4}{\textperiodcentered{}multiply}\PHGap%
\PHToken{FAE8E8}{\textperiodcentered{}both}\PHGap%
\PHToken{F8DEDE}{\textperiodcentered{}the}\PHGap%
\PHToken{E3F0E8}{\textperiodcentered{}numerator}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}and}\PHGap%
\PHToken{BFDDCB}{\textperiodcentered{}denominator}\PHGap%
\PHToken{E1EFE7}{\textperiodcentered{}by}\PHGap%
\PHToken{CAE3D4}{\textperiodcentered{}this}\PHGap%
\PHToken{F3CACA}{\textperiodcentered{}conjug}\PHGap%
\PHToken{E5F1EA}{ate}\PHGap%
\PHToken{E2F0E8}{:\textbackslash{}n\textbackslash{}n}\PHGap%
\PHFocus{%
\PHToken{E5F1EA}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}}\PHGap%
\PHToken{FAE9E9}{frac}\PHGap%
\PHToken{FAE9E9}{\{-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{\}\{}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{\}}\PHGap%
\PHToken{FAE7E7}{\textperiodcentered{}=}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}\textbackslash{}}\PHGap%
\PHToken{F0F1F2}{frac}\PHGap%
\PHToken{FAE9E9}{\{}\PHGap%
\PHToken{F0F1F2}{(-}\PHGap%
\PHToken{F0F1F2}{3}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)\}}\PHGap%
\PHToken{FAE9E9}{\{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{FAE9E9}{)\}\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n\textbackslash{}n}\PHGap%
}%
\noindent%
\PHToken{FAE8E8}{---\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\#\#\#}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}Step}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{E5F1EA}{2}\PHGap%
\PHToken{F0F1F2}{:}\PHGap%
\PHToken{EDAFAF}{\textperiodcentered{}Simpl}\PHGap%
\PHToken{F0F1F2}{ify}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}the}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}Den}\PHGap%
\PHToken{F0F1F2}{ominator}\PHGap%
\PHToken{E5F1EA}{\textbackslash{}n\textbackslash{}n}\PHGap%
\PHToken{7FBB97}{\$\$}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{E5F1EA}{(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)(}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{F0F1F2}{i}\PHGap%
\PHToken{F0F1F2}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{E5F1EA}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}-}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}(}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{E5F1EA}{i}\PHGap%
\PHToken{FAE9E9}{)\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}-}\PHGap%
\PHToken{F5D4D4}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{E38383}{i}\PHGap%
\PHToken{F0F1F2}{\textasciicircum{}}\PHGap%
\PHToken{F0F1F2}{2}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F5D2D2}{\textperiodcentered{}-}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{FAE9E9}{(-}\PHGap%
\PHToken{F0F1F2}{1}\PHGap%
\PHToken{F0F1F2}{)}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F2C4C4}{1}\PHGap%
\PHToken{FAE9E9}{\textperiodcentered{}+}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{4}\PHGap%
\PHToken{F0F1F2}{\textperiodcentered{}=}\PHGap%
\PHToken{E5F1EA}{\textperiodcentered{}}\PHGap%
\PHToken{F0F1F2}{5}\PHGap%
\PHToken{F0F1F2}{\textbackslash{}n}\PHGap%
\PHToken{F0F1F2}{\$\$}\PHGap%
\PHToken{FAE9E9}{\textbackslash{}n\textbackslash{}n}\PHGap%
\par\endgroup
\PHMean{\textcolor{PHNegative}{-0.000041}}{-}
}%
\par\noindent\begin{minipage}{\linewidth}
\PHRule
\PHMeta{\textbf{Interpretation:} The boxed rationalization identity is correct. DCSD stays negative, approaching zero under P3; Base and OPSD cross zero. This is sign stability, NOT evidence that DCSD assigns mathematically correct credit.}
\PHMeta{Signal = model(gold prompt) logp - the same Base(no-answer) logp. Colors encode relative support, not correctness. Mean is for the black frame only.}
\PHSource{Context tokens [2821, 2985); selected tokens [2868, 2917). Selected local example, not an overall ranking.}
\end{minipage}\par\endgroup


==> prompt_horizontal/prompt_horizontal_macros.tex <==
% Load once in the preamble. PH does not collide with the older CS or PB macros.
\RequirePackage{xcolor}
\RequirePackage{textcomp}
\RequirePackage{amsmath}
\definecolor{PHInk}{HTML}{202629}
\definecolor{PHGray}{HTML}{586368}
\definecolor{PHRuleColor}{HTML}{DAE0E1}
\definecolor{PHPositive}{RGB}{54,148,92}
\definecolor{PHNegative}{RGB}{217,88,88}
\newlength{\PHModelWidth}
\newlength{\PHColumnWidth}
\newlength{\PHLabelGap}
\newlength{\PHColumnGap}
\newcommand{\PHInit}{%
  \setlength{\PHModelWidth}{.09\linewidth}%
  \setlength{\PHColumnWidth}{.43\linewidth}%
  \setlength{\PHLabelGap}{.015\linewidth}%
  \setlength{\PHColumnGap}{.035\linewidth}%
}
\newcommand{\PHTokenFont}{\fontsize{7.5}{9.5}\selectfont\ttfamily\color{PHInk}}
\newcommand{\PHToken}[2]{{\setlength{\fboxsep}{.3pt}\colorbox[HTML]{#1}{\strut#2}}}
\newcommand{\PHGap}{\hskip .4pt plus .1pt minus .1pt\relax}
\newsavebox{\PHFocusMeasure}
\newcommand{\PHFocus}[1]{%
  \par\vspace{1pt}\noindent
  \begingroup\setlength{\fboxsep}{1pt}\setlength{\fboxrule}{.5pt}%
  \sbox{\PHFocusMeasure}{#1\unskip}%
  \ifdim\dimexpr\wd\PHFocusMeasure+2\fboxsep+2\fboxrule\relax>\linewidth
    \fbox{\begin{minipage}{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}%
      \PHTokenFont\rightskip=0pt plus 1fil\parfillskip=0pt\noindent#1\unskip\par
    \end{minipage}}%
  \else
    \fbox{\usebox{\PHFocusMeasure}}%
  \fi
  \endgroup\par\vspace{1pt}\noindent\ignorespaces
}
\newcommand{\PHRow}[3]{%
  \par\noindent
  \begin{minipage}[t]{\PHModelWidth}\vspace{0pt}\raggedright\small\bfseries\strut #1\end{minipage}%
  \hspace{\PHLabelGap}%
  \begin{minipage}[t]{\PHColumnWidth}\vspace{0pt}#2\end{minipage}%
  \hspace{\PHColumnGap}%
  \begin{minipage}[t]{\PHColumnWidth}\vspace{0pt}#3\end{minipage}\par
}
\newcommand{\PHColumnTitle}[1]{{\fontsize{8}{10}\selectfont\bfseries\raggedright #1\par}}
\newcommand{\PHTitle}[1]{\par{\normalsize\bfseries\color{PHInk}#1\par}\nobreak\vspace{4pt}}
\newcommand{\PHMeta}[1]{\par{\fontsize{8}{10}\selectfont\raggedright\emergencystretch=2em\color{PHInk}#1\par}\vspace{2pt}}
\newcommand{\PHSource}[1]{\par{\fontsize{8}{10}\selectfont\raggedright\color{PHGray}#1\par}}
\newcommand{\PHRule}{\par\vspace{4pt}{\color{PHRuleColor}\hrule height .4pt}\nobreak\vspace{3pt}}
\newcommand{\PHMean}[2]{\par\vspace{3pt}{\fontsize{7.5}{9.5}\selectfont\ttfamily mean #1\quad[#2]\par}}
\newcommand{\PHLegend}{\PHMeta{%
  \textcolor{PHPositive}{\rule{5pt}{5pt}} Positive\quad
  \textcolor{PHNegative}{\rule{5pt}{5pt}} Negative\quad
  Black frame: selected span. Shared saturation: 0.1 nat.}}


==> prompt_horizontal/prompt_texts_01.tex <==
\begingroup
\PHTitle{Exact user prompts: case 1}
\PHMeta{\textbf{P1}}
\PHMeta{Let \$p(x)\$ be a polynomial of degree 5 such that \textbackslash{}\allowbreak{}[p(n) =\allowbreak{} \textbackslash{}\allowbreak{}frac\{\allowbreak{}n\}\allowbreak{}\{\allowbreak{}n\textasciicircum{}\allowbreak{}2 -\allowbreak{} 1\}\allowbreak{}\textbackslash{}\allowbreak{}]for \$n =\allowbreak{} 2,\$ 3, 4, \$\textbackslash{}\allowbreak{}dots,\$ 7.  Find \$p(8).\$ Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Here is a reference solution: The correct final answer is \textbackslash{}\allowbreak{}frac\{\allowbreak{}3\}\allowbreak{}\{\allowbreak{}56\}\allowbreak{}.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P2}}
\PHMeta{Let \$p(x)\$ be a polynomial of degree 5 such that \textbackslash{}\allowbreak{}[p(n) =\allowbreak{} \textbackslash{}\allowbreak{}frac\{\allowbreak{}n\}\allowbreak{}\{\allowbreak{}n\textasciicircum{}\allowbreak{}2 -\allowbreak{} 1\}\allowbreak{}\textbackslash{}\allowbreak{}]for \$n =\allowbreak{} 2,\$ 3, 4, \$\textbackslash{}\allowbreak{}dots,\$ 7.  Find \$p(8).\$ Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Reference solution for this problem: The correct final answer is \textbackslash{}\allowbreak{}frac\{\allowbreak{}3\}\allowbreak{}\{\allowbreak{}56\}\allowbreak{}.}
\PHMeta{After reviewing the reference solution, solve the problem with your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P3}}
\PHMeta{Here is a reference solution: The correct final answer is \textbackslash{}\allowbreak{}frac\{\allowbreak{}3\}\allowbreak{}\{\allowbreak{}56\}\allowbreak{}.}
\PHMeta{Let \$p(x)\$ be a polynomial of degree 5 such that \textbackslash{}\allowbreak{}[p(n) =\allowbreak{} \textbackslash{}\allowbreak{}frac\{\allowbreak{}n\}\allowbreak{}\{\allowbreak{}n\textasciicircum{}\allowbreak{}2 -\allowbreak{} 1\}\allowbreak{}\textbackslash{}\allowbreak{}]for \$n =\allowbreak{} 2,\$ 3, 4, \$\textbackslash{}\allowbreak{}dots,\$ 7.  Find \$p(8).\$ Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\endgroup


==> prompt_horizontal/prompt_texts_02.tex <==
\begingroup
\PHTitle{Exact user prompts: case 2}
\PHMeta{\textbf{P1}}
\PHMeta{Let \$\textbackslash{}\allowbreak{}triangle ABC\$ have circumcenter \$O\$ and incenter \$I\$ with \$\textbackslash{}\allowbreak{}overline\{\allowbreak{}IA\}\allowbreak{}\textbackslash{}\allowbreak{}perp\textbackslash{}\allowbreak{}overline\{\allowbreak{}OI\}\allowbreak{}\$, circumradius \$13\$, and inradius \$6\$. Find \$AB\textbackslash{}\allowbreak{}cdot AC\$. Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Here is a reference solution: The correct final answer is 468.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P2}}
\PHMeta{Let \$\textbackslash{}\allowbreak{}triangle ABC\$ have circumcenter \$O\$ and incenter \$I\$ with \$\textbackslash{}\allowbreak{}overline\{\allowbreak{}IA\}\allowbreak{}\textbackslash{}\allowbreak{}perp\textbackslash{}\allowbreak{}overline\{\allowbreak{}OI\}\allowbreak{}\$, circumradius \$13\$, and inradius \$6\$. Find \$AB\textbackslash{}\allowbreak{}cdot AC\$. Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Reference solution for this problem: The correct final answer is 468.}
\PHMeta{After reviewing the reference solution, solve the problem with your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P3}}
\PHMeta{Here is a reference solution: The correct final answer is 468.}
\PHMeta{Let \$\textbackslash{}\allowbreak{}triangle ABC\$ have circumcenter \$O\$ and incenter \$I\$ with \$\textbackslash{}\allowbreak{}overline\{\allowbreak{}IA\}\allowbreak{}\textbackslash{}\allowbreak{}perp\textbackslash{}\allowbreak{}overline\{\allowbreak{}OI\}\allowbreak{}\$, circumradius \$13\$, and inradius \$6\$. Find \$AB\textbackslash{}\allowbreak{}cdot AC\$. Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\endgroup


==> prompt_horizontal/prompt_texts_03.tex <==
\begingroup
\PHTitle{Exact user prompts: case 3}
\PHMeta{\textbf{P1}}
\PHMeta{William Sydney Porter tried to perform the calculation \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}-\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}\$. However, he accidentally missed the minus sign, finding \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}=\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}11\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}-\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}2\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}i\$. What answer should he have obtained? Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Here is a reference solution: The correct final answer is 1+\allowbreak{}2i.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P2}}
\PHMeta{William Sydney Porter tried to perform the calculation \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}-\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}\$. However, he accidentally missed the minus sign, finding \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}=\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}11\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}-\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}2\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}i\$. What answer should he have obtained? Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Reference solution for this problem: The correct final answer is 1+\allowbreak{}2i.}
\PHMeta{After reviewing the reference solution, solve the problem with your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P3}}
\PHMeta{Here is a reference solution: The correct final answer is 1+\allowbreak{}2i.}
\PHMeta{William Sydney Porter tried to perform the calculation \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}-\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}\$. However, he accidentally missed the minus sign, finding \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}=\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}11\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}-\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}2\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}i\$. What answer should he have obtained? Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\endgroup


==> prompt_horizontal/prompt_texts_04.tex <==
\begingroup
\PHTitle{Exact user prompts: case 4}
\PHMeta{\textbf{P1}}
\PHMeta{Compute \$17\textasciicircum{}\allowbreak{}\{\allowbreak{}-\allowbreak{}1\}\allowbreak{}\textbackslash{}\allowbreak{}pmod\{\allowbreak{}83\}\allowbreak{}\$. Express your answer as a residue from \$0\$ to \$82\$, inclusive.}
\PHMeta{(You may find it helpful to consider the fact that \$17\textbackslash{}\allowbreak{}cdot 5=\allowbreak{}85\$.) Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Here is a reference solution: The correct final answer is 44.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P2}}
\PHMeta{Compute \$17\textasciicircum{}\allowbreak{}\{\allowbreak{}-\allowbreak{}1\}\allowbreak{}\textbackslash{}\allowbreak{}pmod\{\allowbreak{}83\}\allowbreak{}\$. Express your answer as a residue from \$0\$ to \$82\$, inclusive.}
\PHMeta{(You may find it helpful to consider the fact that \$17\textbackslash{}\allowbreak{}cdot 5=\allowbreak{}85\$.) Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Reference solution for this problem: The correct final answer is 44.}
\PHMeta{After reviewing the reference solution, solve the problem with your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P3}}
\PHMeta{Here is a reference solution: The correct final answer is 44.}
\PHMeta{Compute \$17\textasciicircum{}\allowbreak{}\{\allowbreak{}-\allowbreak{}1\}\allowbreak{}\textbackslash{}\allowbreak{}pmod\{\allowbreak{}83\}\allowbreak{}\$. Express your answer as a residue from \$0\$ to \$82\$, inclusive.}
\PHMeta{(You may find it helpful to consider the fact that \$17\textbackslash{}\allowbreak{}cdot 5=\allowbreak{}85\$.) Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\endgroup


==> prompt_horizontal/prompt_texts_05.tex <==
\begingroup
\PHTitle{Exact user prompts: case 5}
\PHMeta{\textbf{P1}}
\PHMeta{William Sydney Porter tried to perform the calculation \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}-\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}\$. However, he accidentally missed the minus sign, finding \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}=\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}11\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}-\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}2\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}i\$. What answer should he have obtained? Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Here is a reference solution: The correct final answer is 1+\allowbreak{}2i.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P2}}
\PHMeta{William Sydney Porter tried to perform the calculation \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}-\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}\$. However, he accidentally missed the minus sign, finding \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}=\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}11\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}-\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}2\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}i\$. What answer should he have obtained? Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{Reference solution for this problem: The correct final answer is 1+\allowbreak{}2i.}
\PHMeta{After reviewing the reference solution, solve the problem with your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\PHMeta{\textbf{P3}}
\PHMeta{Here is a reference solution: The correct final answer is 1+\allowbreak{}2i.}
\PHMeta{William Sydney Porter tried to perform the calculation \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}-\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}\$. However, he accidentally missed the minus sign, finding \$\textbackslash{}\allowbreak{}frac\{\allowbreak{}3+\allowbreak{}4i\}\allowbreak{}\{\allowbreak{}1+\allowbreak{}2i\}\allowbreak{}=\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}11\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}-\allowbreak{}\textbackslash{}\allowbreak{}frac\{\allowbreak{}2\}\allowbreak{}\{\allowbreak{}5\}\allowbreak{}i\$. What answer should he have obtained? Please reason step by step, and put your final answer within \textbackslash{}\allowbreak{}boxed\{\allowbreak{}\}\allowbreak{}.}
\PHMeta{After understanding the reference solution, solve the problem using your own reasoning. Put the final answer on its own last line in the form `Answer: value`.}
\endgroup

